Flow Correlator: A Flow Table Cache Management Strategy

Switching, routing, and security functions are the backbone of packet processing networks. Fast and efficient processing of packets requires maintaining the state of a large number of transient network connections. In particular, modern stateful firewalls, security monitoring devices, and software-defined networking (SDN) programmable dataplanes require maintaining stateful flow tables. These flow tables often grow much larger than can be expected to fit within on-chip memory, requiring a managed caching layer to maintain performance. This paper focuses on improving the efficiency of caching, an important architectural component of the packet processing data planes. We present a novel predictive approach to network flow table cache management. Our approach leverages a Hashed Perceptron binary classifier as well as an iterative approach to feature selection and ranking to improve the reliability and performance of the data plane caches. We validate the efficiency of the proposed techniques through extensive experimentation using real-world data sets. Our numerical results demonstrate that our techniques improve the reliability and performance of flow-centric packet processing architectures.

==> 0-introduction.tex <==
\chapter{INTRODUCTION}
\label{chap:intro}

% Improve Data Plane processing techniques
% Hardware Optimizations for Data Planes
% Resilience to Denial of Service (Pre-Classification)
% Flow Table cache management (Flow Correlation)

% driving forces
The design-space of network devices is constantly evolving, driven by the continual demand for increased global inter-connectivity, intelligent orchestration, and distribution of computation between cloud and edge resources.
Modern businesses are increasingly reliant on a connected world for a competitive advantage as well as essential operations.
Additionally, there is an increasing urgency to improve the security of critical infrastructure, emphasizing the importance of reliable devices and ultimately resilient networks.


\section{Packet Processing Architectures}
Researchers and industry continue to push the boundaries of packet processing performance and device reconfigurability.
Trade-offs in performance, flexibility, and programmability are being explored with the aim of improving efficiency, reliability, and overall quality of networks.
Networking hardware and software is notably complex, accompanied a high barrier to entry.
It is also difficult, while notably important to guarantee performance across diverse network scenarios.

% processing architectures
Packet processing devices and frameworks trade-off programmability with target performance, ranging from networking ASICs \cite{metamorph, p4}, network processors \cite{mellanox-nps}, to general purpose systems \cite{openvswitch}.
A common architectural advantage of network processors is to provide hardware-assisted event scheduling and table lookup extensions for both on-chip and memory-backed tables.
Many network functions require large flow tables, often consisting of millions of entries and managed across both on-chip and off-chip table resources \cite{fpga-classification}.
To meet performance and cost requirements, caching mechanisms are often employed.
Caching a flow table using on-chip table resources preserve memory bandwidth and reduce latency, but introduces the complexity of effective cache management.



% sdn
\section{Software Defined Networking}
Software Defined Networking (SDN) is an exploration into the formal separation of control plane and data plane constructs.
Motivations include commoditization of data plane hardware (commonly referred to as whitebox switches), reconfigurable flexibility, and longer device life-cycles through software updates and a third party network function application ecosystem.
% Applications can be written on top of the control plane.
% Network Function Virtualization (NFV)
There has been simultaneous resistance and desire to integrate SDN capabilities into networking devices \cite{pof}.
OpenFlow \cite{onf} is a recent effort towards standardizing abstractions and control protocols for data plane manipulation.
Abstractions introduced by this distributed model require careful engineering to reduce associated overheads \cite{tiny}.
% OpenFlow's abstractions also aren't sufficient many devices.

SDN has demonstrated utility, particularly as a diagnostic tool for complex network operations \cite{gu-sdn-forensics}.
The complexities inherent in customizing data plane processing is out of reach to all but the largest enterprises.
The complexity of the constructing SDN systems is notably higher than that of the traditional systems \cite{sdn-security}.
In particular, it is difficult to verify data plane modification do not result in unintended consequences \cite{sdn-consistency, maple}.
In practice, data plane programmability can introduce data paths that violate protocol definitions and various expectation across networking standards \cite{netkat, netcore, wripe}. 
Moreover, SDN applications present unique safety challenges above and beyond traditional programming language libraries and run-times \cite{ frenetic, nettle, arbiter, packet-programs}.

% Recent trends of growing complexity in network hardware place more stress on 
% maybe you can just make the point in a sentence at the end that SDN and other recent trends of growing complexity in router hardware place more stress on the networking hardware and make it more important to accelerate packet processing.



% classification
\section{Packet Classification}
Packet classification is a fundamental component of networking hardware, generally growing in complexity with network size \cite{li2003}.
It is well known that packet classification is expensive and this is a well studied problem in the traditional network hardware domain \cite{gupta2001_hicut, gupta2001, Srinivasan1999, efficuts}.
Complexity of packet classification remains a processing bottleneck, especially in the context of SDN \cite{sdn-classification, ml-classification}.

% security devices rely on classification.  classification is inherently complex.

% target applications?
% two components of many security devices, including stateful firewalls
% It is common for firewalls have access control lists (ACLs) with thousands of matching rules.
% Stateful tracking of transiting flows to ensure adherence to policies as well as auditing


% complexity
Networking devices have a long history of highly specialized designs along with notable service-based market segmentation.
Partly due to the complexity of underlying protocols, but also intricacies involved with ensuring a device meets reliability expectations.
Researchers and enterprises have long been experimenting with trade-offs of increasing the exposed programmability of networking devices.
Specialized applications will continue to demand the ability to categorize, filter, and manipulate flows in increasingly complex ways.
% This is mitigated by specialized architectures leveraging Ternary Content Addressable Memories (TCAMs), Tries, hash, and lookup tables.


% security
% Potential to improve reliability, performance, and intelligent adaptability in network orchestration.

As network reachability and uptime becomes increasingly crucial to modern infrastructure and safety, it is necessary to develop architectural techniques to reduce the impact of Denial-of-Service (DoS).
Not limited to hosted services, underlying network infrastructure is also often vulnerable to DoS \cite{spamhaus}.

Non-uniform processing requirements are a prime target for DoS.
Packet classification is inherently complex with variable processing requirements.
Worse yet, Access Control Lists (ACLs) tend to be focused around allow lists with unauthorized traffic tending to require full ACL traversal, opening the door for DoS attacks on classification.
Accordingly there is a critical need to explore architectures that can improve the resilience of networks.


% perforamnce through caching
Switching and routing functions are a backbone of all networks; however, an increasing number of network functionality requires tracking flow state for transiting connections.
Modern stateful firewalls, security monitoring devices, and corporate edge services rely on efficient implementations of stateful flow tables.
These flow tables often grow much larger than can be expected to fit within on-chip memory, requiring a managed caching layer to meet capacity and performance requirements \cite{flowcache}.
Depending on the network function and performance target, the flow table and caching layers may be distributed across both hardware and software components.
Complicating observability, this caching layer is often obfuscated and embedded between the logical control and data plane layers \cite{sdn-flow-tables}.



% Caching is an important component of many network devices.


%%%%%%%%%%
% \subsection{citations}
% OpenFlow \cite{openflow,openflow_spec} began the networking
% community's embrace of open, platform-independent mechanisms to
% dynamically program network devices.
% OpenFlow \cite{openflow_spec} provided a means to expose predefined tables structures through a protocol specification.
% OpenFlow defines a set of supported protocol headers and actions to manipulate and forward packets in a data plane.
% Several recent works attempt to address scalability and manageability concerns accompanying OpenFlow \cite{openstate, inspired, kandoo, flowcache}.


% General Purpose Software \cite{openvswitch}
% Network Processors (hardware accelerated) tables and task dependency tracking/scheduling \cite{mellanox-nps}.
% Field Programmable Network Pipelines (FPGA, P4) \cite{p4, p4_spec}.
% Networking ASICs \cite{metamorph}.
% Flowcache \cite{flowcache}.
% crazy paper that talks about programs in packets? \cite{packet-programs}.


% Other research and development continues to push for programmable data plane
% constructs and archtectures.
% P4 \cite{p4, p4_spec} is a
% protocol-independent, high-level language for network processors.  P4
% targets flexible variations of fixed-function ASIC switches, often
% referred to as configurable match-action pipelines or Programmable
% Independent Switch Architecture (PISA) \cite{metamorph}.
% The P4 pipeline model begins with a series of programmable parsers
% that extract all headers and fields into a parsed representation;
% then match+action table lookup is performed using this information.

% further complicated by the desire for generic processing abstractions for pogrammable network data planes.

% Table lookups are the most significant part of most data planes, need additional techniques to optimize.


\section{Dissertation Statement}
% Title: Flow Table Management in Programmable Network Data Planes

% Unify a common thread amongst:
% \begin{itemize}
% \item Improve techniques for data plane processing.
% \item Caching in network data planes is notoriously fragile.
% \item Patterns exist in network traffic, yet patterns are noisy.
% \item Room for improvement of cache management algorithms in network devices using pattern based predictors.
% \end{itemize}

% Goal of research is improve performance and reliability through architectural improvements.
% This dissertation presents techniques to improve the reliability and performance of network hardware.
% Architectural techniques to improve the performance and reliability of network devices.
% Temporal patterns are present and crucial to improving performance and reliability of network devices.

\emph{Hardware techniques leveraging temporal patterns can be used to improve the performance and reliability of packet processing architectures.}



\section{Contributions}
% I would add a couple sentences about your approach to the problem after the dissertation statement.  Something like:
In this dissertation we examine how stochastic and speculative hardware techniques can be used to further leverage temporal locality in order to improve performance over existing networking hardware.
% Temporal patterns present in packet inter-arrival patterns provide crucial hints improving performance and reliability of network devices.
The goal of this research is to improve the performance and reliability of packet processing systems through architectural techniques.

\noindent The contributions of this dissertation are summarized as follows:
\begin{enumerate}[i.]
\item Novel use of a stochastic data structure to decouple the impact of malicious packets on established flows.
\item Design and evaluation of a DDoS mitigation strategy to protect classification pipelines with non-uniform execution paths.
  % \item A combined architectural approach that protects established flows from DoS/DDoS.
  % \item A simulation study to evaluate the dynamics of an SDN data plane under attack.
\item Flow table cache management limit study using Belady's MIN on CAIDA network exchange traffic.
\item Application of the Hashed Perceptron binary classifier to network flow table cache management.
\item Iterative approach to feature selection and ranking in the context of Hashed Perceptron binary classifiers.
% in order to improve overall predictor information gain.
% stability under varying network conditions.
\item Discussion of feature roles, granting further perspective into the dynamics of a Hashed Perceptron binary classifier.
\end{enumerate}


\section{Dissertation Organization}
Chapter \ref{chap:preclassification} introduces \emph{Stochastic Pre-Classification}, an architectural technique to harden network functions against Distributed Denial-of-Service (DDoS).
Chapter \ref{chap:caching} advances stateful flow table cache management, introducing \emph{Flow Correlator}, a feature-driven temporal flow activity prediction mechanism.
Finally, Chapter \ref{chap:conclusions} wraps up this dissertation reviewing conclusions and notable future work.




==> abstract.tex <==
\begin{abstract}
    
The design-space of network devices is constantly evolving, driven by the continual demand for increased global inter-connectivity, intelligent orchestration, and distributed computation between cloud and edge resources.
Modern businesses are increasingly reliant on a connected world for a competitive advantage as well as essential operations.
Meanwhile, there is an increasing number of attacks on critical communication infrastructure from a variety of malicious actors.
Thus, there is an increasing urgency to improve all aspects of security in data communication networks.

Additionally, Software-Defined Networking (SDN) has increasingly gained traction and utility across data centers and network administration.
SDN concepts enable increased flexibility for network operators, including the ability to implement a broad class of custom network functions for real-time diagnostics as well as traffic management.
While SDN has notable advantages over traditional network appliances, current implementations are often more susceptible to malicious attacks due to increased complexity and abstractions imposed on packet classification and table management.

This dissertation investigates architectural techniques to improve the reliability and performance of data plane processing hardware.
Our techniques are applicable to both traditional packet processing as well as SDN data plane architectures.
The contributions of this research include two novel and complementary techniques to improve data plane performance through optimizing the use of available packet classification resources.
By leveraging storage-efficient stochastic data structures and machine learning inspired replacement policies, our techniques improve data plane processing efficiency and predictability.

The first technique leverages a Bloom Filter to prioritize established traffic and prevent malicious starvation of expensive packet classification resources.
This \emph{Pre-Classification} technique is general enough to be considered for any classification pipeline with non-uniform processing requirements.
The second technique, originally developed for speculative microprocessors, adapts the Hashed Perceptron binary classifier to flow table cache management.
The proposed \emph{Flow Correlator} mechanism leverages the Hashed Perceptron to correlate flow activity with temporal patterns and transport/network layer hints.
This technique demonstrates the viability of associating temporal patterns to network flows enabling improvements in flow table cache management.
Amenable to hardware implementations, both \emph{Flow Correlator} and \emph{Pre-Classification} techniques show promise in improving the reliability and performance of flow-centric packet processing architectures.
\end{abstract}




==> hp-design.tex <==

\section{Design} \label{sec:hp-design}
One of the goals of this work is to explore a generalized approach to flow table cache management.
Stateful flow tables are core components in the classification pipeline for firewalls and edge security devices.
However, caching can be applied generically to any large table supporting a classification pipeline.
While the focus of this chapter is on improving cache management for stateful flow tables, the techniques we propose can be applied to assist any data plane table considered for caching.

%%%%%%% briefly recap classification?
\begin{figure}[ht]
\centering
\includegraphics[width=0.8\linewidth]{hp_classification} 
\caption{Data Plane Classification Processing}
\label{fig:hp-classification}
\end{figure}

% Data plane processing conceptually consists of multiple table selections, flow selection, and action application cycles to perform the desired network functions.
Figure \ref{fig:hp-classification} portrays an abstract cycle of table selection, flow selection, and action application as the underlying fundamental classification abstraction.
Network functions are composed by chaining multiple logical rounds of classification across relevant flow-state tables.
Network functions that also manipulate packets often also queue data plane and packet actions\footnote{OpenFlow specifies certain actions apply immediately, while others may be queued in an action-set with notable complications.}.
Fundamentally, SDNs aim to expose table management and packet manipulation for a composable packet processing pipeline.
% Intricate details of SDNs (a balance driven by piratical hardware concerns) are out of scope for this exploration.


% \begin{figure}[ht]
% \centering
% \includegraphics[width=\linewidth]{design3} 
% \caption{Data Plane with Flow Cache}
% \label{fig:hp-flow-cache}
% \end{figure}

% Figure \ref{fig:hp-flow-cache} depicts a classification data plane pipeline with an integrated flow cache.
% This figure hints at the potential benefit of including a flow cache.
% However, the complexities of cache are omitted..
% Expanding on the Chapter \ref{chap:preclassification}


%%%%%% describe flow cache management
\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{hp_flow-cache} 
\caption{Flow Cache Management}
\label{fig:hp-flow-cache}
\end{figure}

Figure \ref{fig:hp-flow-cache} shows a classification pipeline focused around a flow cache and a backing stateful flow table.
% Hits in the flow cache are the optimization target fast-path 
It is useful to reiterate that a stateful flow table often resides in off-chip memory due to the number of concurrent flows tracked.
Stateful flow tables are managed by the control plane and a cache is often instantiated in the data plane to meet performance requirements.
There are two high-level scenarios encountered in stateful flow table management:
\begin{itemize}
\item \textbf{New Flow:} Requires classification and a new reservation in the stateful flow table.
\item \textbf{Existing Flow:} Track flow state in relevant table entry for associated packet.
\end{itemize}

A flow cache and its management algorithm must then contend with three scenarios triggered by incoming packets:
\begin{itemize}
\item \textbf{Compulsory Miss:} \emph{New flow}, not yet tracked in the stateful flow table.
\item \textbf{Capacity/Conflict Miss:} \emph{Existing flow}, not currently cached.
\item \textbf{Cache Hit:} \emph{Existing flow}, cached.
\end{itemize}

Cache management algorithms consist of two distinct components: the insertion and replacement policy.
A dynamic insertion policy may choose to bypass cache insertion if the flow is predicted to have a low probability of reuse before eviction.
In networking, bypassing flows based on static protocol heuristics is somewhat common, for example ICMP messages.
However, there is additional opportunity for an insertion algorithm to bypass tracked flows that have a low probability of cache reuse.
Both bypass and early replacement require a means to estimate reuse probability.

Additionally, a dynamic replacement policy may choose to evict a cache entry earlier than a static replacement policy otherwise would.
Since static replacement policies grant all entries equal opportunity for reuse, some flow entries are stuck waiting for eviction, taking up valuable cache resources even when the probability for reuse is markedly lower.
Dynamic replacement policy with an early eviction mechanism provides an additional opportunity to improve cache efficiency by removing stale entries sooner.

% new flow
A packet without an associated flow table entry is considered a new flow, requiring classification.
% Before a flow table entry can be reserved, the flow must first be classified.
Once the flow is classified, the a flow table entry is reserved and the cache management algorithm may be consulted on whether to cache the entry (insert or bypass).
From the perspective of the flow cache, new flows triggering classification are compulsory misses -- an unavoidable slow-path.
% Classifying flows and updating flow tables are the most computationally intensive events.

% existing flow, cache miss
Once a flow is tracked by the stateful flow table, the classification pipeline no longer needs to be consulted.
However, the effectiveness of the limited cache resources is ultimately up to the cache management algorithm.
This design aims to minimize the cache misses encountered by existing flows by exploring better cache management techniques.

% existing flow, cache hit
Packets that encounter hits in the flow cache may simply update the cached flow table entry without needing to access off-chip flow table resources.
A more intelligent cache management algorithm has the potential to significantly improve the flow cache hit-rate and thus data plane processing performance. 
% Through improving the cache management algorithm, 

%%%%% detail flow cache management algorithm?

% \begin{itemize}
% \item \textbf{Existing Flow (Hit):} Replacement policy may keep or mark for early eviction.
% \item \textbf{New Flow (Compulsory Miss:} Insertion policy may bypass or insert.
% \item \textbf{Existing Flow (Capacity/Conflict Miss):} Insertion policy may bypass or insert.
% \end{itemize}


%%%%% finish with introduction of flow correlator; augment the existing baseline cache management


The remaining section outlines the design details of the flow correlator mechanism.
Apart from design-time feature selection, the hashed perceptron flow correlation approach does not require global weight training.
The hashed perceptron feedback mechanism resembles an online training technique, adjusting correlation tables dynamically at run-time.

%%%% section organization...?
The adaptation of hashed perceptron cache management as a flow correlation mechanism is described in Section \ref{sec:hp-hp-design}.
As with many machine learning approaches, selecting useful Features at design-time is non-trivial and requires artful exploration.
Our approach to feature design and metrics are covered in Section \ref{sec:hp-selection}.
Since feature selection consumed a majority of our effort during design iteration, we developed an iterative optimization approach generically applicable to tuning Hashed Perceptron based cache management.
Section \ref{sec:hp-information-gain} describes this methodical approach to approximating information gained by differential performance analysis.



\subsection{Classifier Metrics} \label{sec:hp-classifier-metrics}
Early in feature exploration, we heavily leveraged average and standard deviations of both pure and mixed features to help gain insight into input sparsity.
However, simply analyzing input and output distributions alone isn't sufficient to distinguish predictive features.

Analysis of binary classification problems is well studied, applicable across many research domains.
The aptly named \emph{Confusion Matrix} is commonly used to summarize the behavior of binary-outcome systems.
Table \ref{tab:hp-confusion-matrix} depicts a common representation of a confusion matrix.

% \emph{True Positive}
% which elaborates all possible prediction scenarios of a binary classifier.
% The \emph{actual} ground truth represented as row and columns representing \emph{predictions}.

\begin{table}[H]
\centering
\begin{tabular}{lcccl}
 & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textit{Predicted}} &  \\ \cline{3-4}
 & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{Negative} &  \\ \cline{2-4}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{\cellcolor{pastelG}True Positive} & \multicolumn{1}{c|}{\cellcolor{pastelR}False Negative} &  \\ \cline{2-4}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textit{Actual}}} & \multicolumn{1}{c|}{Negative} & \multicolumn{1}{c|}{\cellcolor{pastelR}False Positive} & \multicolumn{1}{c|}{\cellcolor{pastelG}True Negative} &  \\ \cline{2-4}
\end{tabular}
\caption{Confusion Matrix}
\label{tab:hp-confusion-matrix}
\end{table}


While simple ratio metrics are heavily used in certain domains, they aren't sufficiently robust for this work.
\emph{Accuracy} (Eq. \ref{eq-accuracy}) considers both positive and negative cases; however it is easily swayed by even moderately unbalanced datasets.
The \emph{F1} score (Eq. \ref{eq-f1}) is similarly unsuited as it is essentially \emph{accuracy} focused only on the positive set -- used primarily as a positive detection metric.

% \begin{itemize}
% \item Correlation Matrix imprecise for selection decision, but gives hints about shared information.
% \item Accuracy, Precision only half the picture due to unbalanced binary classes
% \end{itemize}

\begin{equation} \label{eq-accuracy}
accuracy = \frac{TP+TN}{TP+TN+FP+FN}
\end{equation}

\begin{equation} \label{eq-f1}
F1 = \frac{2 TP}{2 TP+FP+FN}
\end{equation}



% \subsubsection{Matthew's Correlation Coefficient} \label{sec:hp-mcc}
Matthew's Correlation Coefficient (MCC) is a particularly useful metric to compare binary classifier performance \cite{matthews1975}.
MCC (Eq. \ref{eq-mcc}) is derived from Pearson's correlation coefficient applied specifically to binary classification.
MCC provides a balanced view of the confusion matrix, reducing decision bias from skewing the perceived accuracy.
Appendix \ref{appendix:mcc} provides further intuition on the interpretation of MCC as defined in Equation \ref{eq-mcc}
% MCC effectively scales the accuracy contributed by the prediction instances, providing a weighted notion of actual contribution.

% is less sensitive to data imbalances, employing all four entries within the confusion matrix. If the confusion matrix entries are divided by the total number of experiential measurements, m = TP+TN+TN+FN, the numerical entries approximate the underlying two-dimensional joint-probability distribution function (discrete probabilities).

\begin{equation} \label{eq-mcc}
MCC = \frac{TP*TN - FP*FN}{\sqrt{(TP+FP)(TP+FN)(TN+FP)(TN+FN)}}
\end{equation}

% MCC is bound between -1 and 1. As the MMC approaches +1, the predictor approaches excellent performance in a  "positive logic" sense. As the MCC approaching -1, the predictor approaches an excellent predictor, but in a "negated logic" sense (always wrong, so negating the prediction is required).  When the MCC is near 0 demonstrating no correlation between predictions and actual data. data.  

As a correlation coefficient, MCC is bound between $-1$ and $1$. 
A positive MCC indicates a correlation to correct predictions; while a negative MCC indicates anti-correlation.
An MCC near zero indicates a weak correlation, hinting at a poor prediction confidence resembling a random process.
As MCC approaches $\pm 1$, the predictor is deemed to have a relatively higher prediction confidence.
Ultimately MCC provides a balanced view of binary classifier performance, particularly useful when operating within reasonable bias limitations \cite{chicco-mcc, Zhu-mcc-imbalance}.


\begin{table*}[b]
\centering
\begin{tabular}{lcccl}
 & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textit{Predicted}} &  \\ \cline{3-4}
 & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Active} & \multicolumn{1}{c|}{Dormant} &  \\ \cline{2-4}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Active} & \multicolumn{1}{c|}{\cellcolor{pastelG} Active Correct (TP) } & \multicolumn{1}{c|}{\cellcolor{pastelR} Dormant Incorrect (FN) } &  \\ \cline{2-4}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textit{Actual}}} & \multicolumn{1}{c|}{Dormant} & \multicolumn{1}{c|}{\cellcolor{pastelR} Active Incorrect (FP) } & \multicolumn{1}{c|}{\cellcolor{pastelG} Dormant Correct (TN) } &  \\ \cline{2-4}
\end{tabular}
\caption{Flow Correlation Confusion Matrix}
\label{tab:hp-confusion-matrix-2}
\end{table*}


To assist in subsequent sections, Table \ref{tab:hp-confusion-matrix-2} specializes the confusion matrix around predictions of flow activity in the context of cache management.
Section \ref{sec:hp-reinforcement} will connect each case in the confusion matrix to the hashed perceptron training algorithm.


\subsection{Flow Correlator Design} \label{sec:hp-hp-design}
% Just a highlevel overview of how your scheme works.  Include high-level block digram of the system.

% Design-time tuning for performance under expected network conditions.
% Design decisions to improve robustness to unusual operating conditions.
% Because of the resemblance of the hashed perceptron mechanism to perceptron in the machine learning field, many researchers ...

% The Hashed Perceptron structure maps input feature-space to binary classes.
The hashed perceptron technique provides a structured mechanism to leverage multiple prediction tables for improved overall accuracy and resiliency.
The hashed perceptron training algorithm plays a crucial role in keeping these predictor tables balanced across multiple features.
Apart from design-time feature selection, the hashed perceptron flow correlation approach does not require global weight training.
The hashed perceptron feedback mechanism resembles an online training technique, adjusting correlation tables dynamically at run-time.

The hashed perceptron consists of correlation tables (feature tables) consulted during inference.
Each correlation table is indexed by a feature and contains saturating counters (weights) resembling typical prediction tables.
The Hashed Perceptron differs from single-perspective predictors by combining the predictions from multiple feature tables to produce a final combined decision.
The magic of the hashed perceptron centers around the ability to manage multiple tables cohesively using a prediction feedback mechanism (the hashed perceptron training algorithm).

% While every flow transiting the device will result in a flow table entry, a subset of the most active flows will reside in a flow table cache.
Flow table cache management relies on accurately predicting reuse for a given flow.
This ultimately boils down to predicting packet inter-arrival patterns for each active Flow.
More specifically, predicting the likelihood of a subsequent packet arrival for a given flow within the relative time window allotted by the cache's working set.

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.7\linewidth]{hp-structure} 
% \caption{Flow Correlator Overview}
%\label{fig:hp-overview}
% \end{figure}

The Hashed Perceptron mechanism is conceptually split into two phases: inference and reinforcement.
Section \ref{sec:hp-inference} describes the process of generating a reuse prediction for every packet arrival.
Section \ref{sec:hp-reinforcement} describes the Hashed Perceptron training algorithm as the basis for maintaining prediction tables.


\subsubsection{Inference} \label{sec:hp-inference}
Cache management predictions are generated in real-time by the flow correlator inference mechanism.
%%%%%%%%% Setup by introducing processing requirements?
Every packet event triggers an inference prediction for cache management, thus it is crucial that inference is able to meet the packet processing requirement of the underlying design target.
% Inference essentially consists of parallelizable feature table is one of the primary advantages of the hashed perceptron mechanism
% One of the advantages of the hashed perceptron structure is.
% On every cache lookup, the hash perceptron is consulted prediction 


% two prediction types; same inference pipeline
Cache management handles two scenarios depending on the cached state of the flow entry.
First, a flow cache miss triggers a cache management decision to insert or bypass the flow entry.
% Entries already inserted into the cache
% The cache management context changes to an early eviction Flow cache hits 
Secondly, cache management seeks to identify optimal scenarios for early eviction.
An early eviction, or conversely a reuse prediction, is performed on a flow cache hit.
In both scenarios, cache management consults flow correlation inference to estimate the likelyhood of flow entry reuse relative to overall cache pressure.
% The flow correlator inference pipeline is identical for both bypass as well as early eviction predictions.

Both predictions are essentially re-framing an underlying flow entry reuse prediction around a relative ranking of flow activity.
Thus, the flow correlator inference and training pipelines are organized around the concept of \emph{active} or \emph{dormant} flows.
Both bypass and early eviction share table resources, interpreting positive table weights as likely to be \emph{active} and negative weights as likely \emph{dormant}.
% It is important to note that the overall flow correlator predictor is conceptually organized around active/dormant flows, the feature tables are correlation mappings from observable feature patterns into indicators of active/dormant flows.
% However, features themselves do not track flow state.

\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{hp_inference} 
\caption{Flow Correlator Inference}
\label{fig:hp-inference}
\end{figure}

%%%%%% Walk through inference steps
Figure \ref{fig:hp-inference} outlines the flow correlator's inference pipeline.
%%%%%%%%% Talk about assembling features:
In order for cache management to generate an inference, the feature components must first be gathered from the packet header bitfields and the relevant flow table entry.
Stateless protocol feature components originate from the packet headers and are readily available by preexisting classification \emph{Key Extraction} operations.
Stateful feature components (e.g. burstCount) are pulled from a cached flow table entry during a cache hit, or simply zero during a cache miss.

%%%% lookup, threshold, prediction
Each assembled feature ($f_{N*}$) indexes into a corresponding feature table providing a mapping to independent correlations ($C_{N*}$).
The decision threshold ($\theta$) is applied to the sum of each feature's correlation.
Since $\theta$ is zero for this flow correlator design, the magnitude of the accumulated correlations can be interpreted as a confidence and the sign represents the decision.
% These correlations are accumulated across each feature and thresholded by the decidion threshold ($\theta$).
%($|<\!C_{N*}\!>|$)
% A reuse prediction is made by summing all feature correlations together and finally thresholding.

% A flow with corresponding extracted features producing a positive combined correlation is interpreted as likely to see reuse.
% Conversely, a negative combined correlation is interpreted as dormant within the current available working set of the cache.

On inference, each feature contributes an opinion as a correlation count.
The hashed perceptron structure accumulates the correlations from all features, thresholding to create a reuse prediction.
The confidence of the feature's opinion, can be inferred by the magnitude of the correlation count.
Similarly, the confidence of the overall prediction is the magnitude of all accumulated correlations.

% Focusing on inference itself, this figure assumes packet bit-fields are already extracted and assembled into the appropriate relevant features.
% The Active/Dormant prediction history queues will be discussed in Section \ref{sec:hp-reinforcement}.
% Ultimately bypass is a reuse prediction, differing only in that the flow table entry is not currently cached.
% It is important to conceptually distinguish bypass from reuse as a designer during feature selection.


% Hashed Perceptron consists of Feature tables, consisting of saturating counters as well as prediction delay queues used for training feedback.
% Each prediction table consists of small saturating counters, representing the correlation weight.



%%%%%%%%% Feature Table sizes..
Feature tables map a disjoint input feature-space to cache reuse correlations.
Loosely resembling a hash, features are often orthogonal combinations of several bit fields.
% Each assembled feature indexes into a corresponding feature table.
These feature table lockups are performed in parallel.
Each feature table holds saturating correlation counters, commonly referred as weights.
Each feature table's length is $2^{m}$ entries where $m$ refers to the bit-width of the corresponding feature assembly.
The implementation requirements of each feature is then simply $w * 2^{m}$ bits, where $w$ refers to the saturating counter bit-width.



% Cache Hit -> Reuse? (Predict flow is active) -> keep in cache
% Cache Hit -> Reuse? (Predict flow is inactive) -> mark for early eviction
% Cache Miss -> Bypass? (Predict flow is active) -> insert into cache
% Cache Miss -> Bypass? (Predict flow is inactive) -> bypass cache

%%%%% Discuss intracacies of early eviction...
Flow entries marked for early eviction by the flow correlation mechanism are in the cache, but prioritized for replacement.
When a flow entry needs to be inserted and no entries are marked for early eviction, replacement falls back to LRU.
If a flow entry marked for early replacement encounters a hit before eviction, the prediction is corrected and a training event is triggered.


\subsubsection{Reinforcement} \label{sec:hp-reinforcement}
% The hashed perceptron mechanism relies on an online training algorithm organized around a prediction feedback loop.
The hashed perceptron mechanism consists of an online training algorithm organized around prediction feedback.
Applied to flow correlation, prediction feedback seeks correlations of flow entry reuse across feature vectors.
With respect to the available cache resources, the flow correlation predictor aims to rank flow entries by likelihood of reuse within the available cache working set.

% Ultimately, correlation state is spread across feature tables, where the weights... 

%%%%%%% introduce feedback mechanism:
% The feedback delay is implicit in the length of the prediction history queues, used to mimic the cache delay itself.
 % relative to the design's nominal cache pressure.
% and by leveraging a delay feedback loop.


\emph{Active} flow predictions are inserted into the active history queue, while \emph{dormant} flow predictions are inserted in the dormant history queue.
In order to reinforce cache management decisions, these feedback queues must be searchable by a unique flow identifier.
The flow identifier implementation leveraged by the flow cache may be borrowed for this purpose.

%%%%%%% Future work...?
%%%%%%% Prediction history queue depths are a design optimization parameter
% Feedback queues are searchable by a tag of corresponding flow table entry's flow identifer (flowID).
% The full 5-tuple flow identifier (flowID) was used in this exploration; however, a lightweight flowID mixing technique can be leveraged at the cost of potential false positives identifying flow reuse.


%%%%%%% two scenarios for active prediction: correct/incorrect
% The confusion matrix in Figure \ref{tab:hp-confusion-matrix-2}
Hashed perceptron training reinforcement consists of four potential scenarios, each corresponding to entries in the confusion matrix.
\emph{Active} prediction reinforcement is shown in Figure \ref{fig:hp-training-tp} and Figure \ref{fig:hp-training-fp} covering the \emph{true positive} and \emph{false positive} cases, respectively.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\linewidth]{hp_training_tp} 
\caption{Active Correct (TP) Reinforcement}
\label{fig:hp-training-tp}
\end{figure}

In Figure \ref{fig:hp-training-tp}, the example flow $F_{3}$ has a prior \emph{active} flow prediction awaiting confirmation in the \emph{active history} queue.
Since the prior reuse prediction is now proved correct, the feature vector, $\langle f_{3} \rangle$, associated with the previous prediction is popped off of the queue.
If the prediction confidence associated with $\langle f_{3} \rangle$ do not surpass the training threshold, the corresponding feature table correlation counts are incremented.
The new reuse prediction associated with $F_{3}$ is also pushed into the \emph{active history} queue along with the associated new feature vector, $\langle f_{3*} \rangle$.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\linewidth]{hp_training_fp} 
\caption{Active Incorrect (FP) Training}
\label{fig:hp-training-fp}
\end{figure}

Figure \ref{fig:hp-training-fp} outlines how incorrect \emph{active} flow predictions are determined.
Example flow $F_{N}$ does not have a previous reuse prediction, yet is predicted active by inference.
% This situation occurs when flow $F_{N}$ is new or otherwise \emph{dormant}, now predicted \emph{active}.
In order to free a slot, the oldest prediction is popped off the end of the \emph{active history} queue and considered incorrect.
The example flow $F_{1}$ and feature table correlation counts associated with feature vector $\langle f_{1} \rangle$ are decremented.
Note the training threshold is omitted since the \emph{active} flow prediction associated with $F_{1}$ was determined to be incorrect.
The new reuse prediction associated with $F_{N}$ is pushed into the \emph{active history} queue along with its feature vector, $\langle f_{N*} \rangle$.


%%%%%% two scenarios for dormant prediction:
The next two figures illustrate \emph{dormant} flow prediction reinforcement covering the \emph{true negative} and \emph{false negative} cases of the confusion matrix, respectively.
Conversely to \emph{active history}, entries popped off the end of the \emph{dormant history} queue are considered correct.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\linewidth]{hp_training_tn} 
\caption{Dormant Correct (TN) Reinforcement}
\label{fig:hp-training-tn}
\end{figure}

Figure \ref{fig:hp-training-tn} illustrates example flow $F_{N}$ predicted \emph{dormant} during inference.
Finding no prior prediction associated with $F_{N}$, the oldest prediction in the \emph{dormant history} queue is popped off the end.
% Since the prior \emph{dormant} prediction associated with $F_{1}$ is correct, the training threshold is consulted.
% Conversely to \emph{active history}, predictions popped off the end of the \emph{dormant history} queue are considered correct.
% associated with $F_{1}$ is considered correct.
If the prediction confidence associated with $\langle f_{1} \rangle$ do not exceed the training threshold, the corresponding feature table correlation counts are decremented -- reinforcing the correct \emph{dormant} prediction.
The new \emph{dormant} prediction associated with $F_{N}$ is pushed into the \emph{dormant history} queue along with its feature vector, $\langle f_{N*} \rangle$.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\linewidth]{hp_training_fn} 
\caption{Dormant Incorrect (FN) Training}
\label{fig:hp-training-fn}
\end{figure}

In Figure \ref{fig:hp-training-fn}, the example flow $F_{3}$ has a prior \emph{dormant} flow prediction awaiting confirmation in the \emph{dormant history} queue.
The prior \emph{dormant} prediction was caught before falling off the end of the queue, indicating that feature vector $\langle f_{3} \rangle$ may contain hints towards flow reuse.
The existing $F_{3}$ entry and associated feature vector, $\langle f_{3} \rangle$, is removed from the queue and the respective feature table correlation counts incremented.
Note once again that the training threshold is omitted since the \emph{dormant} flow prediction associated with $F_{3}$ was determined to be incorrect.
Finally, the new reuse prediction associated with $F_{3}$ is pushed into the \emph{dormant history} queue along with the associated new feature vector, $\langle f_{3*} \rangle$.


% final reiteration between reinforcement vs training?
% make clear that every packet must search both \emph{active} and \emph{dormant} prediction history queues for reinforcement.
% however, the new prediction is inserted into \emph{active} or \emph{dormant} based on its prediction.
% note: diagrams do not quite showcase edge case of current/past prediction differing.


%%%%%  talk about simplifying of thresholds:
% Many specialized applications of the Hashed Perceptron have opted include optimizing decision and training threshold as yet another design parameter.
Seznec developed a dynamic training thresholding mechanism for the GEometric History Length branch predictor \cite{seznec-thresholding}.
% Seznec's adaptive mechanism proved valuable in eliminating both thresholds as design parameters in our flow correlation design.
We leveraged Seznec adaptive mechanism for the \emph{training threshold} ($\Phi$), which also requires the \emph{decision threshold} ($\theta$) to be centered around zero.
% can be dynamically adjusted to balance predictor aggressiveness.
Through experimentation, we confirmed that Seznec's target $1\!:\!1$ ratio of correct to incorrect predictions resulted in the best overall predictor accuracy, matching our experimentally tuned parameters.

While the optimal $\Phi$ depends on the cache pressure, we observed a notably stable threshold once the predictor warmed up and aggressiveness balanced.
It is also notably advantageous to keep the decision threshold ($\theta$) intuitively at zero -- preserving the numeric symmetry of weights as well as accumulated correlations.
% The influence metric he weights and a analysis advantage when


% \begin{enumerate}
% \item Design parameter: determining how long to validate incorrect prediction before reinforcing as a correct prediction.
% \item Update frequency considerations: 1:1 with inferences?  potential for sampling, but trades off work for latency to update.  (we chose 1:1 for this work, with fixed-depth indexed fifo queues for delay loop).
% \end{enumerate}




\subsection{Feature Design} \label{sec:hp-selection}
Table \ref{tbl:hp-all-features} lists features explored during the design process with remarks on approximate intent behind each combination.
There is limited information available from fields contained within each packet.
However, we found notable value in associating temporal patterns with hints from packet fields.
The features outlined in this table are nowhere near an exhaustive exploration, but rather a first pass to identify useful combinations.


\begin{table*}[t]
\centering
\singlespacing
\begin{tabular}{clll}
% \begin{tabular}{cllp{0.35\linewidth}}
\textbf{$f_{\#}$} & \textbf{Feature Type} & \textbf{Feature Components} & \textbf{Remarks} \\
0  & Control & $UniformRandom$ & Uncorrelated: map to random entry \\
1  & Pure Mix & $ipProto \wedge min(srcPort, dstPort)$ & Protocol hints \\
2  & Pure Mix & $ipv4Dst[31\!\colon\!16] \wedge dstPort$ & Destination service \\
3  & Pure Mix & $ipv4Src[31\!\colon\!16] \wedge srcPort$ & Source service \\
4  & Pure & $flags$ & TCP/IP flags \\
5  & Pure & $srcPort \wedge dstPort$ & Bi-directional TCP/UDP ports \\
6  & Pure Mix & $f_{TCP}\!\ll\!7 \wedge f_{1}$ & Mix TCP flags with protocol hint \\
7  & Pure & $(ipv4Dst \wedge ipv4Src)[31\!\colon\!16]$ & Bi-directional upper 16-bits IP addresses \\
8  & Pure & $(ipv4Dst \wedge ipv4Src)[23\!\colon\!8]$ & Bi-directional middle 16-bits IP addresses \\
9  & Pure & $(ipv4Dst \wedge ipv4Src)[15\!\colon\!0]$ & Bi-directional lower 16-bits of IP addresses \\
% 7  & Pure & $Upper16(ipv4Dst) \wedge Upper16(ipv4Src)$ & Bi-directional upper 16-bits IP addresses \\
% 8  & Pure & $Middle16(ipv4Dst) \wedge Middle16(ipv4Src)$ & Bi-directional middle 16-bits IP addresses \\
% 9  & Pure & $Lower16(ipv4Dst) \wedge Lower16(ipv4Src)$ & Bi-directional lower 16-bits of IP addresses \\
10 & Pattern & $\lceil flowPackets \rceil_{16}$ & Packets since start of flow \\
11 & Pure & $ipLength$ & IP frame length \\
12 & Pure & $flowID$ & 5-tuple flow identifier \\
13 & Pure Mix & $f_{12} \wedge f_{11}$ & Unroll frame length over flowID \\
14 & Pattern & $\lceil refCount \rceil_{16}$ & Hit count while inserted into cache \\
15 & Pattern & $\lceil burstCount \rceil_{16}$ & Hit count while in MRU position \\
16 & Pattern Mix & $\{ \lceil f_{14} \rceil_8, \lceil f_{15} \rceil_8 \}$ & Concatenate RefCount and BurstCount \\
17 & Pure + Pattern & $f_{16} \wedge f_{12}$ & Unroll Burst/RefCount over flowID \\
18 & Pure + Pattern & $f_{16} \wedge f_{7}$ & Unroll Burst/RefCount over upper IP \\
19 & Pure + Pattern & $f_{16} \wedge f_{8}$ & Unroll Burst/RefCount over middle IP  \\
20 & Pure + Pattern & $f_{16} \wedge f_{9}$ & Unroll Burst/RefCount over lower IP \\
21 & Pure + Pattern & $f_{11} \wedge f_{7}$ & Unroll frame length over upper IP \\
22 & Pure + Pattern & $f_{11} \wedge f_{8}$ & Unroll frame length over middle IP  \\
23 & Pure + Pattern & $f_{11} \wedge f_{9}$ & Unroll frame length over lower IP \\
24 & Pure Mix & $ipFragOffset \wedge f_{4} \wedge f_{11} \wedge f_{12}$ & \makecell[l]{Unroll fragment offset, flags, and \\frame length over flowID} \\
25 & Pure Mix & $f_{7} \wedge f_{4}$ & Unroll flags over upper IP \\
26 & Control & $NULL$ & Sparsity: map to single entry\\
27 & Pure + Pattern & $\{f_{11}, \lceil f_{15} \rceil_8 \}$ & Concatenate BurstCount with frame length \\
28 & Pure + Pattern & $f_{16} \wedge f_{11}$ & Unroll Burst/RefCount over frame length
\end{tabular}
\longcaption{Complete List of Explored Features}{
% \caption*{\textmd{ 
Concatenation syntax is represented as $\{A, B\}$.
$\lceil A \rceil_N$ refers to the ceiling function: $min(A, N)$.
The XOR operation is indicated by $\wedge$.
$A\!\ll\!N$ represents left shift left by N-bits.
Bit-field selection is indicated using the syntax $[M\!\colon\!N]$, where bit positions $M$ through $N$ are extracted.}
\label{tbl:hp-all-features}
\end{table*}


% You need a para setting up the next 3 subsubsub sections, stating what the different types of features are before diving into them. 

The \emph{Feature Type} column approximately categorizes each feature by information sources.
There are two potential sources of information: \emph{Pure} (stateless) and \emph{Pattern} (stateful).
Pure feature components originate from packet headers.
Pattern feature components introduce temporal information, not already available within packet headers.
\emph{Pure Mix} are simple combinations of packet header bit-fields.
\emph{Pattern Mix} refers to combinations of temporal state.
Finally, \emph{Pure + Pattern} are combinations of both packet header bit-fields and temporal state.
Appendix \ref{appendix:features} provides all feature table weight distributions for comparison alongside the descriptions below.

% Features that allow for early indication of reuse improve effective bypass performance?
% Features that track access patterns improve early evict performance?
% A tricky aspect of feature design is understanding when features beneficent from being generalized vs spread out by flow.
% Often found generalized features performed best under low cache pressure.



\subsubsection{Pure Features} \label{sec:hp-pure-features}
There are really only five pure feature components originating from packet headers explored in this study.
These include IP source and destination addresses, IP protocol identifier, TCP/UDP port numbers, IP frame length, and few grouped IP/TCP flags.
The IP flags assembled in $f_{4}$ are: DF and MF.
The TCP flags assembled in $f_{4}$ and $f_{6}$ are: SYN, FIN, RST, PSH, ACK, URG. 
% and in f6?
% While some pure features performed well, the system preferred combinations

% Double check me.....


\subsubsection{Temporal Pattern Features} \label{sec:hp-pattern-features}
Pattern features are distinguished from Pure features as they require temporal metadata in the flow table entry.
These pattern feature components do not originate from packet headers, but offer the ability to associate sequences or temporal patterns between packets.
Pattern based featured proved to be valuable sources of information, but required mixing to unlock their potential.
% Packet count, $f_{10}$, is likely already tracked by the backing flow table and present in a cached flow table entry.

The flowPackets feature ($f_{10}$) is simply the packet count since the flow started, a counter often already present in stateful flow tables.
RefCount ($f_{14}$) and BurstCount ($f_{15}$) on the other hand are similar counters, but unique to the lifetime of the cached flow table entry.
RefCount is simply the packets observed since the flow was inserted into the cache, while BurstCount is the packets observed while the entry remains in the MRU position.
% Further details are provided in Section \ref{sec:hp-stack}.



% \subsubsection{Feature Combinations}
\subsubsection{Combined Features}
There are endless ways to assemble features with complementary pure and pattern-based components.
There were two conceptual approaches when attempting to constructively combine features components: \emph{orthogonal combination} and \emph{correlation unrolling}.

\emph{Orthogonal combinations} allows for better utilization of feature table resources through a union of independent feature components.
For example: some feature components are useful for bypass predictions, while others provide hints toward early eviction.
Usually we observed a trade-off in feature information density at the cost of collisions and reduced confidence.
However, we also observed potential for coincidental benefit -- correlations simultaneously occurring, strengthening feature confidence.
% Additionally, we observed a non-trivial trade-off between feature-space density and 
% However there is a tradeoff as feature components are inherently noisy.

\emph{Feature unrolling}, as an approach towards enabling constructive feature combinations aiming to distribute global correlations across subsets of flow designators such that opportunities for independent correlations may arise.
% Feature unrolling is a means to spread out differentiating feature mapping across multiple entries in hopes of discovering common correlations within subsets.
For example: temporal patterns tend to perform better when associated with partial IP address subsets, protocol, or port designators.
Correlation unrolling is a balance and can either benefit or detract from feature performance.

Pattern-based features are particularly complex in the context of networking.
Subsets of flows may exhibit similar patterns, but all flows together tend to be quite noisy with conflicting inter-arrival patterns.
Thus, we observed notable utility in correlating pattern-based feature components across protocol differentiating components.
It is also important to conceptualize that each packet in a given flow maps to different flow table entries throughout the sequence.
The inter-arrival access patterns is thus encoded across multiple entries in any given table.
% When a feature input correlates to a significant indicator of flow entry reuse, the entry will increase...
% Entries without much correlation will stay around 0...

There is certainly a trade-off ranging from targeting independent per-flow correlations to strategic groupings sharing correlator entries.
Unlike bloom filter designs where hashes are desired to be as uniquely identifying and free of collisions as possible, 
there is a balance in hashed perceptron feature construction where carefully selected subsets improve correlation potential.

The designer can choose to combine orthogonal features, or unroll features by spreading potential correlations out over subsets of flows.
Since necessary unrolling can increase a features effective training latency, there is a non-obvious trade-off between the concept of sharing correlations across subsets of flows as well as enabling flows to maintain independent correlations.
The features presented in this work are almost certainly non-optimal, but do provide insight towards successful (as well as unsuccessful) combinations.

% Potential to combine multiple prediction questions into one hashed perceptron structure (trade-off of collisions vs. shared space).  Does this space compression behave like Bloom Filters?  (We choose to simply combine Bypass and Early Eviction into one structure as they are similar in premise)


\subsubsection{Control Features} \label{sec:hp-control-features}
To help understand the natural bias of the system, two control features were included in the study: UniformRandom ($f_{0}$) and NULL ($f_{26}$).
These were only used in the feature exploration process as a likeness comparison
UniformRandom simply chooses a table entry randomly based on a uniform random distribution, providing insight into the hysteresis of the system.
NULL is effectively a single table entry (5-bit saturating counter), representing sparse feature behavior.

Combining too many components reduces the opportunities for correlations.
We have observed that heavily mixed features, such as features that combine the full flow identifier (flowID, $f_{12}$) tend to under-perform features that combine a partial flow identifier such as $f_{7}$.
All components mixed together into a single feature tends to approach UniformRandom ($f_{1}$) while sparse features tend to resemble NULL ($f_{26}$).



%%%%%%%%
\subsection{Feature Metrics} \label{sec:hp-feature-metrics}
Since the hashed perceptron structure consists of multiple independent prediction tables contributing opinions towards an overall prediction, there is a need to analyze feature performance relative to the overall system.
Just as MCC is a notably useful classifier metric, it can also be calculated with respect to each feature, independently.
% Tracking prediction confirmations both for the overall predictor as well as each feature independently.
% classifier metrics can be applied to individual features.
 % of accuracy, such as MCC.


% discuss how actual is calculated in the context of the simulation.  
The Hashed Perceptron training feedback is assumed to be ground truth.
Absolute truth is non-trivial to ascertain as each misprediction has implications that propagate forward in time.
% As the Hashed Perceptron 
Imperfect, ground truth is a practical compromise that extends to all feature analysis techniques in this work.

% The confusion matrix is calculated as follows:
% table/matrix with TP, FP, TN, FN mapped to predictions?


% \subsubsection{Feature Correlation} \label{sec:hp-feature-correlation

% Observations:
% - Correlation between features vs. correlation to correct decision
% - Solo vs. Combined features - spreading information in a useful way (de-aliasing? unrolling?)
% -- e.g. Trade-off in attempting to correlate global burst-count patterns vs spreading out to many indepdentent patterns



\subsubsection{Feature Influence} \label{sec:hp-influence}
% You want to get at here why you came up with this metric and what its aim is before you discuss how you calc it
% This is an important part of your work, I think you want to make this a subsection with a discussion of why you need a new metric to evaluate features.

While MCC is well suited for relative feature comparisons, it doesn't quite grant insight into the confidence of predictions.
Specifically in the context of the hashed perceptron mechanism, each feature has the potential to influence the system prediction equally.
However well behaved features self-moderate their confidence by the weight of their contribution.
 % -- interpreted as the feature's confidence.
Understanding how a feature contributes to the overall system provides valuable feedback into the behavior of feature components as well as intuition into successful combinations.


\begin{table}[H]
\centering
\begin{tabular}{lcccl}
%%% Pweight notation
%  & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textit{Predicted}} &  \\ \cline{3-4}
%  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{Negative} &  \\ \cline{2-4}
% \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{\cellcolor{pastelG} $\frac{\sum \vec{P}_{weight}}{TP}$ } & \multicolumn{1}{c|}{\cellcolor{pastelR} $\frac{\sum \vec{P}_{weight}}{FN}$ } & \\[1mm] \cline{2-4}
% \multicolumn{1}{c|}{\multirow{-2}{*}{\textit{Actual}}} & \multicolumn{1}{c|}{Negative} & \multicolumn{1}{c|}{\cellcolor{pastelR} $\frac{- \sum \vec{P}_{weight}}{FP}$ } & \multicolumn{1}{c|}{\cellcolor{pastelG} $\frac{- \sum \vec{P}_{weight}}{TN}$ } &  \\[1mm] \cline{2-4}
% \\

%%% fweight notation
%  & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textit{Predicted}} &  \\ \cline{3-4}
%  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{Negative} &  \\ \cline{2-4}
% \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{\cellcolor{pastelG} $\frac{\sum \vec{f}_{weight}}{TP}$ } & \multicolumn{1}{c|}{\cellcolor{pastelR} $\frac{\sum \vec{f}_{weight}}{FN}$ } & \\[1mm] \cline{2-4}
% \multicolumn{1}{c|}{\multirow{-2}{*}{\textit{Actual}}} & \multicolumn{1}{c|}{Negative} & \multicolumn{1}{c|}{\cellcolor{pastelR} $\frac{- \sum \vec{f}_{weight}}{FP}$ } & \multicolumn{1}{c|}{\cellcolor{pastelG} $\frac{- \sum \vec{f}_{weight}}{TN}$ } &  \\[1mm] \cline{2-4}
% \\

% %%% w_f notation
 & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textit{Predicted}} &  \\ \cline{3-4}
 & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{Negative} &  \\ \cline{2-4}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{\cellcolor{pastelG} $\frac{\sum \vec{w}_f }{TP}$ } & \multicolumn{1}{c|}{\cellcolor{pastelR} $\frac{\sum \vec{w}_f }{FN}$ } & \\[1mm] \cline{2-4}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textit{Actual}}} & \multicolumn{1}{c|}{Negative} & \multicolumn{1}{c|}{\cellcolor{pastelR} $\frac{- \sum \vec{w}_f}{FP}$ } & \multicolumn{1}{c|}{\cellcolor{pastelG} $\frac{- \sum \vec{w}_f}{TN}$ } &  \\[1mm] \cline{2-4}
\\

%%% C_f notation
%  & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textit{Predicted}} &  \\ \cline{3-4}
%  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{Negative} &  \\ \cline{2-4}
% \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Positive} & \multicolumn{1}{c|}{\cellcolor{pastelG} $\frac{\sum \vec{C}_f }{TP}$ } & \multicolumn{1}{c|}{\cellcolor{pastelR} $\frac{\sum \vec{C}_f }{FN}$ } & \\[1mm] \cline{2-4}
% \multicolumn{1}{c|}{\multirow{-2}{*}{\textit{Actual}}} & \multicolumn{1}{c|}{Negative} & \multicolumn{1}{c|}{\cellcolor{pastelR} $\frac{- \sum \vec{C}_f}{FP}$ } & \multicolumn{1}{c|}{\cellcolor{pastelG} $\frac{- \sum \vec{C}_f}{TN}$ } &  \\[1mm] \cline{2-4}

\end{tabular}
\caption{Influence Matrix}
\label{tab:hp-influence-matrix}
\end{table}


Table \ref{tab:hp-influence-matrix} shows how influence is an extension of the confusion matrix.
The influence matrix is categorized with respect to the overall correctness of the system prediction (TP, TN, FP, FN).
The vector notation simply indicates that feature weights ($\vec{w_f}$) are accumulated independently, with respect to each system prediction.
% while the corresponding weights of each feature are accumulated with respect to the system decision.

Note that influence of a single-feature predictor is simply the average weight with respect to that predictor's confusion matrix.
However, the influence metric becomes more than just an average weight when per-feature contributions are tracked with respect overall system decisions.
% More precisely, the influence matrix prediction accounting (TP, TN, FP, FN) is tracked with respect to the overall system decision; while the corresponding weights of each feature are accumulated with respect to the system decision.
Influence grants insight into the feature's contribution, or lack thereof, relative to the correctness of the system's overall prediction.

Influence can be analyzed with respect to each quadrant of the confusion matrix.
As noted above, the influence vector notation $\vv{I\!N\!F}$ indicates individual per-feature weight accumulations ($\vec{w}_f$) with respect to system decisions.
To simplify analysis, feature influence can be grouped with respect to correct and incorrect system predictions.

\begin{equation}
% influence_{correct} = \frac{\sum P_{weight}}{TP} - \frac{\sum P_{weight}}{TN}
\vv{I\!N\!F}_{correct} = 
\frac{\displaystyle\sum^{T\!P} \vec{w}_f}{TP} - 
\frac{\displaystyle\sum^{T\!N} \vec{w}_f}{TN}
\label{eq:f-correct-inf}
\end{equation}

Equation \ref{eq:f-correct-inf} defines \emph{Correct Influence} as the contributed weight towards correct decisions.
The numerical value of correct influence is the average weight contributed towards correct predictions.
Correct Influence can be interpreted as a feature's confidence when deemed correct, providing unique insight alongside prediction accuracy.

\begin{equation}
% influence_{incorrect} = \frac{\sum P_{weight}}{FN} - \frac{\sum P_{weight}}{FP}
\vv{I\!N\!F}_{incorrect} = 
\frac{\displaystyle\sum^{F\!N} \vec{w}_f}{FN} - 
\frac{\displaystyle\sum^{F\!P} \vec{w}_f}{FP}
\label{eq:f-incorrect-inf}
\end{equation}

Similarly, Equation \ref{eq:f-incorrect-inf} defines the \emph{Incorrect Influence} as the contributed weight towards incorrect decisions.
Incorrect influence can be interpreted as a feature's overconfident contribution towards incorrect predictions.
Overconfident features ultimately detract from an otherwise potentially correct prediction, a notably useful insight unique to influence.
To improve interpretation, \emph{Incorrect Influence} maintains the same directionality alongside \emph{Correct Influence}, where weight contributions towards incorrect predictions are negative numeric values, while correct contributions despite being overruled are positive.


% Understanding not just the feature's balanced accuracy (MCC), but also the relative \emph{influence} on the final outcome is notably helpful 
% It is useful to know how opinionated any given feature was towards a prediction (or miss-prediction) in addition to the balanced accuracy granted by MCC.

The negation of the \emph{FP} and \emph{TN} accumulations map all correct predictions into a positive influence and incorrect predictions into negative influence.
Total influence can them be considered the sum of correct and incorrect influence as shown in Equation \ref{eq:f-total-inf}.

\begin{equation}
% influence_{total} = influence_{correct} + influence_{incorrect}
\vv{I\!N\!F}_{total} = \vv{I\!N\!F}_{correct} + \vv{I\!N\!F}_{incorrect}
\label{eq:f-total-inf}
\end{equation}

% A feature's current opinion is represented by the correlation count contained in the feature table for a given feature vector component.
% Influence represents the contribution a feature had towards the final decision.

Ideally, features would remain impartial until sufficient correlation occurs to form a reliable prediction.
In practice, features can be confidently wrong or even marginally correct while still providing value to the system.
Independently, features often produce noisy and inaccurate predictions.
Considered together with the hashed perceptron structure, feature noise is averaged away while simultaneous correlations combine to improve prediction quality.

The notable difference between MCC and Influence centers around the penalty attributed to mispredictions.
MCC treats all feature predictions equally, regardless of the accompanying confidence.
Rather, influence provides a perspective into the confidence towards correct decisions as well as overconfidence towards incorrect decisions.
MCC provides a robust balanced accuracy, where influence grants insight into contributions.
% Correct Hashed Perceptron predictions are often pushed over the decision threshold by confidently correct features that overrule features with less confidence.

Features able to regulate their overconfidence are notably valuable to the system -- even if they only occasionally grant unique perspectives.
% Mispredictions that are accompanied with a properly regulated confidence
While there will inherently be inaccuracies in any history-based pattern correlation mechanism, understanding feature contributions towards correct/incorrect decisions helps during feature selection and tuning.




%%%%%%%%%
\subsubsection{Inferring Information Gain} \label{sec:hp-information-gain}
Information gain has been influential in decision trees \cite{decision-tree-ig} as a tool to estimate mutual information.
% mutual information between two competing nodes
% Relative entropy, formally Kullback-Leibler divergence is a difference measurement between two probability distributions.
Decisions trees leverage information gain as a means to estimate mutual information between competing branches when growing as well as trimming decision trees.

Inspired by information gain, we leverage a similar technique comparing the differential performance gain (or loss) between adjacent simulation runs.
Algorithm \ref{alg:hp-sweep} defines a simulation sweep across an ordered set of features.
By incrementally adding features in ranked order, information gained by the added feature can be estimated through a resulting change in the simulation's performance metric.
% : cache hit-rate, estimated performance, etc.
Plotting the improvement (or degradation) of each additional feature grants insight into any objectively useful information added to the system.

\begin{algorithm}
  \caption{Simulation Feature Sweep}
  \label{alg:hp-sweep}
  \begin{algorithmic}[1]%1: line numbers
    \Function{Sweep}{$\vec{R}$} \funclabel{alg:sweep}
    \Comment{Simulation hit-rate sweep across feature ranking}
      \For{$n \gets 1$ to $\Call{Length}{\vec{R}}$}
        % \Comment{Ranked order from 1 to N features, inclusive}
        \State $\vec{r}\gets \{\vec{R}[0],~...,~\vec{R}[n]\}$
            \Comment{Feature subset to include in simulation run}
        \State $\vec{P}[i]\gets \Call{Simulate}{\vec{r}}$
            % \Comment{Performance of feature subset}
      \EndFor
      \State \Return $\vec{P}$
        \Comment{Simulation performance metric in inclusive ranked order}
      \EndFunction
  \end{algorithmic}
\end{algorithm}

% Both metrics do not take into account shared information.  But we can approximate that with a differential approximation similar to: (insert Random Tree exploration literary work...)
This \emph{feature sweep} estimation is particularly useful as both MCC and influence are inherently unable to identify shared information between competing features.
Realizing that competing rankings can be compared by sweeping features,
 we stumbled on an approach to prune shared information.
 Algorithm \ref{alg:hp-ig-loop} describes our approach to formalize our process of feature ranking in the context of a hashed perceptron prediction system.
  % finding a decent narrow in on a better overall ranking.
% analyzing two competing ranked ordering mechanisms.


% Initial ranking:  MCC
% “Sweep” from 1 to N ranked features
% CacheSimulation(<f1, … ,fN>)
% New ranking:  sort by adjacent difference in speedup
% Repeat step 2 until stable ranking
\begin{algorithm}
  \caption{Differential Information Gain}
  \label{alg:hp-ig-loop}
  \begin{algorithmic}[1]
    % \Function{InitalRank}{$\vec{F}$} \funclabel{alg:initial-mcc}
    % \Comment{Inferring information gain through differential hit-rate improvement}
    %   \State $p\gets \Call{Simulate}{\vec{F}}$
    %   \State $\vec{R}\gets \Call{MCC}{p}$
    %     \Comment{Calculate MCC for each feature}
    %   \State \Return $\vec{R}$
    %     \Comment{Initial ranking determined by MCC}
    % \EndFunction

    \Function{IG}{$\vec{F}$} \funclabel{alg:ig}
    \Comment{Inferring information gain through differential system improvement}
      \State $p_{0}\gets \Call{Simulate}{\vec{F}}$
      \State $\vec{R}_{0}\gets \Call{MCC}{p_{0}}$
        \Comment{Initial ranking provided by MCC}
      \State $i\gets 1$
      \While{$\vec{R}_{i} \not= \vec{R}_{i-1}$}
        \Comment{Repeat until ranking is stable}
        \State $\vec{p}\gets$ \Call{Sweep}{$\vec{R}_{i-1}$}
        \State $\vec{q}\gets \Call{AdjacentDifference}{\vec{p}}$
            \Comment{Calculate relative improvement gain}
        \State $\vec{R}_{i}\gets \Call{Sort}{\vec{q}}$
        \State $i\gets i + 1$
      \EndWhile\label{endloop}
      \State \Return $\vec{R}_{i}$
        \Comment{New ranking sorted by relative improvement}
      \EndFunction
  \end{algorithmic}
\end{algorithm}


Ranking features purely by information gain is tempting, but unfairly favors the features already selected over the differential new feature added.
This algorithm greedily optimizes to the nearest local minimum.
However, this technique is notably useful in eliminating mutual information from an already decent initial feature ranking provided by MCC.






==> hp-efficiency.tex <==
% Warning: PDF inclusion: multiple pdfs with page group included in a single page
% for now, just supress warning as transparancy pallet should always be similar..
\pdfsuppresswarningpagegroup=1


\section{Cache Pressure Dynamics} \label{appendix:efficiency}

%%%%%% Observing Cache Pressure dynamics through Cache Size %%%%%
\begin{longtable}{ccc}
\centering
\includegraphics[width=53mm]{2k-8_clockTimeLast} &
\includegraphics[width=53mm]{4k-8_clockTimeLast} &
\includegraphics[width=53mm]{8k-8_clockTimeLast} \vspace{-10pt}\\
2k, 8-way &
4k, 8-way &
8k, 8-way \\
\caption{Cache Size vs. Entry Lifetime} \\
\end{longtable}

\begin{longtable}{ccc}
\centering
\includegraphics[width=53mm]{2k-8_clockTimeDead} &
\includegraphics[width=53mm]{4k-8_clockTimeDead} &
\includegraphics[width=53mm]{8k-8_clockTimeDead} \vspace{-10pt}\\
2k, 8-way &
4k, 8-way &
8k, 8-way \\
\caption{Cache Size vs. Entry Deadtime} \\
\end{longtable}


\begin{longtable}{ccc}
\centering
\includegraphics[width=53mm]{2k-8_clockTimeEfficiency} &
\includegraphics[width=53mm]{4k-8_clockTimeEfficiency} &
\includegraphics[width=53mm]{8k-8_clockTimeEfficiency} \vspace{-10pt}\\
2k, 8-way &
4k, 8-way &
8k, 8-way \\
\caption{Cache Size vs. Efficiency} \\
\end{longtable}


%%%%%% Associativity's affect on HP's Ranking %%%%%%
\newpage
\begin{longtable}{ccc}
\centering
\includegraphics[width=53mm]{2k-4_clockTimeLast} &
\includegraphics[width=53mm]{4k-4_clockTimeLast} &
\includegraphics[width=53mm]{8k-4_clockTimeLast} \vspace{-10pt}\\
2k, 4-way &
4k, 4-way &
8k, 4-way \\

\includegraphics[width=53mm]{2k-8_clockTimeLast} &
\includegraphics[width=53mm]{4k-8_clockTimeLast} &
\includegraphics[width=53mm]{8k-8_clockTimeLast} \vspace{-10pt}\\
2k, 8-way &
4k, 8-way &
8k, 8-way \\

\includegraphics[width=53mm]{2k-16_clockTimeLast} &
\includegraphics[width=53mm]{4k-16_clockTimeLast} &
\includegraphics[width=53mm]{8k-16_clockTimeLast} \vspace{-10pt}\\
2k, 16-way &
4k, 16-way &
8k, 16-way \\

\caption{Cache Associativity vs. Entry Lifetime} \\
\end{longtable}


==> hp-features.tex <==
% Warning: PDF inclusion: multiple pdfs with page group included in a single page
% for now, just supress warning as transparancy pallet should always be similar..
\pdfsuppresswarningpagegroup=1


\section{Feature Table Weight Distributions} \label{appendix:features}
% \begin{samepage}
% \begin{spacing}{1.5}
% \subsection{Selected Features}

% \vspace*{-5pt}
\begin{longtable}{c}
\begin{tabular}{ccc}
\includegraphics[width=51mm]{2012-sanjose_weight-dist-6} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-27} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-21} \\
\end{tabular} \\
\begin{tabular}{cc}
\includegraphics[width=51mm]{2012-sanjose_weight-dist-18} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-10} \\
\end{tabular} \vspace{-10pt} \\

\shortcaption{Distributions of Selected Features}{in \emph{IG\textsubscript{3}-4k} ranked order} \\
\end{longtable}

% \begin{longtable}{cc}
% % \textbf{$f_{\#}$} & 
% \textbf{Feature Table Weights} & \textbf{Feature Table Inference} \\

% % 6 &
% \includegraphics[width=60mm]{2012-sanjose_weight-dist-6} &
% \includegraphics[width=60mm]{2012-sanjose_inferred-weight-dist-6} \\

% % 27 &
% \includegraphics[width=60mm]{2012-sanjose_weight-dist-27} &
% \includegraphics[width=60mm]{2012-sanjose_inferred-weight-dist-27} \\

% % 21 &
% \includegraphics[width=60mm]{2012-sanjose_weight-dist-21} &
% \includegraphics[width=60mm]{2012-sanjose_inferred-weight-dist-21} \\

% % 18 &
% \includegraphics[width=60mm]{2012-sanjose_weight-dist-18} & 
% \includegraphics[width=60mm]{2012-sanjose_inferred-weight-dist-18} \\

% % 10 &
% \includegraphics[width=60mm]{2012-sanjose_weight-dist-10} &
% \includegraphics[width=60mm]{2012-sanjose_inferred-weight-dist-10} \\
% % (d) & (e) \\[6pt]
% \end{longtable}
% \caption{Selected Feature Distributions}
% In \emph{IG\textsubscript{3}-4k} ranked order.
% \end{figure}

% \vspace*{-5pt}

% \begin{figure}[H]
\begin{longtable}{ccc}
\centering
\includegraphics[width=51mm]{2012-sanjose_weight-dist-7} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-11} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-1} \\

\includegraphics[width=51mm]{2012-sanjose_weight-dist-15} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-16} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-14} \vspace{-10pt} \\

\shortcaption{Distributions of Contributing Feature Components}{in \emph{MCC-4k} ranked order} \\
\end{longtable}
% \end{figure}
% \end{spacing}
% \end{samepage}



% \begin{figure}[H]
\begin{longtable}{ccc}
\centering

\includegraphics[width=51mm]{2012-sanjose_weight-dist-4} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-28} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-22} \\

\includegraphics[width=51mm]{2012-sanjose_weight-dist-25} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-8} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-23} \\

\includegraphics[width=51mm]{2012-sanjose_weight-dist-3} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-9} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-12} \\

\includegraphics[width=51mm]{2012-sanjose_weight-dist-13} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-5} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-2} \\

\includegraphics[width=51mm]{2012-sanjose_weight-dist-24} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-19} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-20} \\

% \includegraphics[width=51mm]{2012-sanjose_weight-dist-17} &
% \includegraphics[width=51mm]{2012-sanjose_weight-dist-0} &
% \includegraphics[width=51mm]{2012-sanjose_weight-dist-26} \vspace{-10pt} \\

\shortcaption{Distributions of Rejected Feature Components}{in \emph{MCC-4k} ranked order}\label{hp-app:rejected-distrbutions} \\

& \includegraphics[width=51mm]{2012-sanjose_weight-dist-17} & \vspace{-10pt} \\

\shortcaptioncontinued{Distributions of Rejected Feature Components}{in \emph{MCC-4k} ranked order}{\ref{hp-app:rejected-distrbutions}} \\

\end{longtable}
% \end{figure}


\begin{longtable}{cc}
\centering
\includegraphics[width=51mm]{2012-sanjose_weight-dist-0} &
\includegraphics[width=51mm]{2012-sanjose_weight-dist-26} \\

\caption{Distributions of Control Features} \\
\end{longtable}

% \begin{figure*}[ht]
% \begin{tabular}{ccc}
% & \includegraphics[width=70mm]{2012-sanjose_weight-dist-1} & \\
% \end{tabular}
% \label{Feature 6 Weight Distribution}
% \end{figure*}


\newpage
\section{Selected Features' Composition} \label{appendix:selected}
% remove extra \newline incured by section (thesis office fix)
\vspace{-\baselineskip}

\begin{figure}[H]
\centering
\includegraphics[width=75mm]{2012-sanjose_weight-dist-27} \\
% \begin{tabular}{cc}
% \includegraphics[width=60mm]{2012-sanjose_weight-dist-11} &
% \includegraphics[width=60mm]{2012-sanjose_weight-dist-15}
% \end{tabular}
\caption{$f_{27}$ Weight Distribution}
\end{figure}

\begin{figure}[H]
\centering
\begin{tabular}{cc}
\includegraphics[width=60mm]{2012-sanjose_weight-dist-11} &
\includegraphics[width=60mm]{2012-sanjose_weight-dist-15} \\
\end{tabular}
\caption{$f_{27}$ Compositions' Weight Distributions}
\end{figure}

\newpage

\begin{figure}[H]
\centering
\includegraphics[width=75mm]{2012-sanjose_weight-dist-21} \\
\caption{$f_{21}$ Weight Distribution}
\end{figure}

\begin{figure}[H]
\centering
\begin{tabular}{cc}
\includegraphics[width=60mm]{2012-sanjose_weight-dist-11} &
\includegraphics[width=60mm]{2012-sanjose_weight-dist-7} \\
\end{tabular}
\caption{$f_{21}$ Compositions' Weight Distributions}
\end{figure}


\newpage
\begin{figure}[H]
\centering
\includegraphics[width=75mm]{2012-sanjose_weight-dist-18} \\
\caption{$f_{18}$ Weight Distribution}
\end{figure}

\begin{figure}[H]
\centering
\begin{tabular}{cc}
\includegraphics[width=60mm]{2012-sanjose_weight-dist-16} &
\includegraphics[width=60mm]{2012-sanjose_weight-dist-7} \\
\includegraphics[width=60mm]{2012-sanjose_weight-dist-14} &
\includegraphics[width=60mm]{2012-sanjose_weight-dist-15} \\
\end{tabular}
\caption{$f_{18}$ Compositions' Weight Distributions}
\end{figure}


% \begin{figure}[H]
% \centering
% \includegraphics[width=75mm]{2012-sanjose_weight-dist-10} \\
% \caption{$f_{10}$ Weight Distribution}
% \end{figure}


% \newpage
% \begin{figure}[H]
% \centering
% \includegraphics[width=75mm]{2012-sanjose_weight-dist-6} \\
% \caption{$f_{6}$ Weight Distribution}
% \end{figure}

% \begin{figure}[H]
% \centering
% \includegraphics[width=60mm]{2012-sanjose_weight-dist-1}
% \caption{$f_{6}$ Composition's Weight Distribution}
% \end{figure}


% \subsection{Explored Features}
% \begin{figure*}[ht]
% \begin{tabular}{ccc}
% \includegraphics[width=51mm]{2012-sanjose_weight-dist-1} &
% \includegraphics[width=51mm]{2012-sanjose_weight-dist-6} &
% \includegraphics[width=51mm]{2012-sanjose_weight-dist-7} \\
% \end{tabular}
% \label{Leveraged Pure Features' Weight Distribution}
% \end{figure*}


% \begin{figure*}[ht]
% \centering
% \begin{tabular}{cc}
% \includegraphics[width=51mm]{2012-sanjose_weight-dist-0} &
% \includegraphics[width=51mm]{2012-sanjose_weight-dist-26} 
% \end{tabular}
% \label{Control Features' Weight Distribution}
% \end{figure*}


==> hp-intro.tex <==

\section{Introduction}
Caching is an important component of many network devices.
Switching and routing functions are a backbone of all networks; however, an increasing amount of network functionality requires maintaining flow state for transiting connections.
Modern stateful firewalls, security monitoring devices, and software defined networking require maintaining stateful flow tables.
These flow tables often grow much larger than can be expected to fit within on-chip memory, requiring a managed caching layer to maintain performance.
This caching layer is often obfuscated and embedded between the control and data plane layers.

The design-space of network devices is continually evolving with trade-offs in performance and reconfigurability.
A common architectural advantage of network processors is to provide hardware-assisted table lookup extensions for both on-chip and memory-backed tables.  % CITEME: mellanox
Network functions requiring large flow tables, often consisting of millions of entries, require managing both on-chip and off-chip table resources.
To meet performance and cost requirements, caching mechanisms are commonly employed.
Caching a flow table using on-chip table resources preserves memory bandwidth and reduces latency, but introduces the complexity of effective cache management.

%However, most of these generic architecutres don't provide hardware-based trasparent caching.
%show distribution of packets vs. flows in CAIDA traces?
% I'd then mention that prior work in processor caching shows that patterns exist in those workloads that allow better than LRU performance.

%Caching is considered critical to modern processor microarchitecture, where decades of research has explored extended or replaced the canonical least-recently used (LRU) replacement algorithm.

%Similarly bypassing, or more generally, insertion priority has also been an important component in order to adapt to streaming conditions.  %where lru fails..?
% cite denning?  

%Well known caching conditions including streaming and thrashing apply to patterns observed in flow table management for network devices.

% You can then mention that you hypothesize that there are patterns in network traffic that could be similarly leveraged.  Your goal with this work is to examine how modern caching policies can improve performance over traditional LRU.
In processor microarchitecture, it has long been known that software inherently exhibits locality that can be leveraged at run-time.
Cache management for network flow tables has historically seen less research interest than in processor microarchitecture.
Insight into state of the art flow table management tends to be particularly shrouded in proprietary implementations.
Existing flow table cache management heuristics are primarily based on the Least Recently Used (LRU) replacement as well as explicit protocol-based bypass mechanisms.

% TODO:
% You probably could have one or two more paras here.  A lot of your work revolved around HP and feature selection.
% You should setup that with a para here mentioning how ML techniques can be used in caching but that feature selection is a critical problem for that.


\subsection{Contributions}
% Inspired by the intricacies observed in packet inter-arrival patterns, 
% This chapter aims to explore if flow table cache management techniques can be improved.

% Leveraging prior works, we highlight an approach to bound expectations of flow table cache hit-rates using an oracle replacement algorithm.
% We highlight our success in applying the hashed perceptron mechanism to flow table cache management.
% Finally, we reflect on our feature design methodology, highlighting feature combinations were most beneficial, as well as insights into future analysis.

This chapter aims to explore if locality in network traffic can be leveraged with more advanced cache management techniques.
We review several modern cache management approaches in microarchitecture, highlighting our progress exploring flow table cache management.
The contributions of this chapter include:

\begin{enumerate}
\item Flow table cache management limit study using Belady's MIN replacement algorithm on CAIDA network exchange traffic.
\item First work to apply a Hashed Perceptron binary classifier to network flow table cache management.
% \item Iterative approach to Hashed Perceptron feature selection and analysis.
\item Iterative approach to feature selection and ranking in the context of Hashed Perceptron binary classifiers.
% \item Observation of feature roles under changing cache pressure dynamics within Hashed Perceptron based cache management.
\item Discussion of feature roles, granting further perspective into the dynamics of a Hashed Perceptron binary classifier.
\end{enumerate}


% TODO: Insert layout paragraph...




%%%%%%%%%%%%%%%%%%%%
\section{Motivation}
% I'd start Background with a subsection on optimal replacement and Belady's.  Including a discussion of what that's not practical.  This can frame the discussion of the other policies as different mechanisms to approach Belady's

To bring perspective to the objective metrics used in this chapter, Section \ref{sec:hp-hit-rate} first describes the significance of cache hit-rate to system performance.
In order to understand the upper bound on room for improvement to cache hit-rate, we start with an optimality study in Section \ref{sec:hp-opt}.
Cacheable packet inter-arrival patterns and their timescales are further motivated in Section \ref{sec:hp-patterns}.
Section \ref{sec:hp-stack} reviews well known stack-based cache management algorithms.
Limitations to traditional approaches adapted to caching in networking are outlined in Section \ref{sec:hp-failures}.
Finally, we wrap up by introducing modern multi-perspective approaches to cache management using the hashed perceptron binary classifier in Section \ref{sec:hp-perceptron}.


\subsection{Significance of Cache Hit-Rate} \label{sec:hp-hit-rate}
System architects need to understand the impacts and potential drawbacks of caching, including estimations of processing latency and throughput.
Caching allows mitigating slow-path processing requirements by taking advantage of locality.
The actual performance benefit of a proposed caching implementation depends on the ability to capture the effective working set available in the workload.
It is important to quickly assess the potential expected performance improvement granted by a proposed caching architecture.

\begin{equation}
APPT \approx AMAT = T_{fast} + Miss Rate \times T_{slow}
\label{equ:f-estimate-performance}
\end{equation}

Equation \ref{equ:f-estimate-performance} rephrases average memory access time (AMAT) to approximate the sensitivity of cache hit-rate on average packet processing time (APPT).
As accumulated packet processing effort roughly tracks processing latency, APPT can be approximated through a first-order processing latency estimation.
In the context of packet processing, $T_{slow}$ represents the average latency (or effort) exerted while traversing the slow-path.
$T_{fast}$ represents the average latency (or effort) consumed when a cache hit enables fast-path processing.
% The $MissRate$ refers to the cache miss-rate, as the complement to hit-rate: $1-HitRate$.
It is expected that the processing effort between fast and slow paths could be an order or two apart -- further motivating the desire to maximize cache hit-rate.

% AMAT and the rephrased APPT are focused around latency; a similar first-order equation can be derived for processing effort to approximate sensitivity to packet processing efficiency.
The wide verity of stateful network functions as well as packet processing architectures make it difficult to settle on a specific known ratio between $T_{fast}$ and $T_{slow}$. 
For simplicity, this first-order sensitivity estimation is scoped to a single data plane packet processing slice.
A more detailed analysis approach may be needed to take into account intricacies of parallel processing pipelines.

% Is predictable hit-rates more important or are we just trying to say misses are bad.  The later is easier to get across:
% Not only is minimizing $MissRate$ crucial to both latency and throughput in any caching system
% , but it is also essential to understand the stability of cache hit-rates under worst-case scenarios

As is common in processor microarchitecture cache management, small percentile average hit-rate improvements often translate into notably significant ten-percentile performance gains.
While the sensitivity estimation is ultimately left to the designer, it is conceivable that single-digit hit-rate improvements presented in this chapter may translate to a multiple-digit performance speedup for stateful network functions reliant on caching.


\subsection{Cache Optimality Study} \label{sec:hp-opt}
Originally developed to study optimal page replacement for virtual memory systems, Belady's Minimal page replacement algorithm (MIN) has been applied to cache replacement in processor microarchitecture \cite{belady-min, belady-replacement, mattison-stack}.
Belady's MIN algorithm effectively orders the replacement stack by next furthest access, maximizing cache hit-rate.

Outside of a few specialized domains with bounded working sets or known access patterns, an optimal replacement ranking is usually impractical to build in hardware.
% Of course, a portal into the future is required to provide this idealized replacement ranking.
% Notable insights can be provided by an oracle replacement algorithm, including an understanding of availible 
Unpredictable random events will be capturable by MIN, but elusive to practical implementations which rely on pattern history.
As an upper bound, Belady's MIN provides useful insight to cache replacement as well as potential headroom to improve cache hit-rate.


\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{min-lru_breakdown}
\longcaption{Belady's MIN Optimal Replacement}{
% Fully associative cache hit-rate simulation bounding improvement between LRU and MIN.\\
% Flow table cache simulation using CAIDA Equinix Sanjose 2012 (equinix-sanjose.20120119).
Fully associative flow table cache hit-rate simulation.  CAIDA Equinix Sanjose January 2012 dataset.}
\label{fig:hp-belady}
\end{figure}

Figure \ref{fig:hp-belady} shows the cache hit-rate for both the oracle Belady's MIN algorithm and a baseline fully-associative LRU implementation.
% Belady's MIN provides an upper bound on the achievable hit-rate, limited only by cache capacity.
While compulsory misses (misses caused by new flows) are unavoidable, MIN's capacity misses are entirely limited by the cache capacity and not also the replacement algorithm.
The hit-rate delta between MIN and LRU is an upper bound to best possible hit-rate improvement achievable by improving the cache management algorithms.

At 4k flow entries, LRU achieved $15.8\%$ fewer hits relative to MIN, with $23.7\%$ true capacity misses remaining.
This gap reduced to $7.2\%$ fewer hits at 64k entries, with only $4.7\%$ capacity misses remaining.
It is expected that there will always be a gap between realistic cache management algorithms and oracle algorithms.
However, the following sections aim to investigate the potential for improvement.

This limit study suggests there might be a potential cacheable working-set \cite{denning-working-set} larger than what LRU is able to capture.
However, there is no guarantee that the gap between MIN and LRU is practically achievable.
Intuitively, MIN also confirms greater potential improvement as cache size decreases.
% small caches in this context are on the order of 4:100 -> 1:25 -> 1 entry / 25 pps...?
Section \ref{sec:hp-performance} further discusses the significance of hit-rate including the expected impact on overall system performance.

% If network traffic is driven strictly by a random process, the gap between MIN and LRU is not achievable in practice.
% Recent research has expanded on the Belady algorithm to also include prefetching \cite{cite-me}.


\subsection{Flow Patterns} \label{sec:hp-patterns}
% In addition to transport layer patterns which are more well understood and modeled, we theorize that network flows also exhibit cacheable patterns driven by program phases on connection endpoints \cite{markov-traffic-modeling}.
While network traffic, particularly transport layer protocol behavior, is relatively well understood and modeled \cite{markov-traffic-modeling};
we theorize that network flows also exhibit locality driven by program phases on connection endpoints.
Examples of side-channel attacks \cite{ssh-sidechannel} further support inherent end-host program behavior embedded within packet inter-arrival patterns.


\begin{figure*}[t]
\centering
% \begin{tabular}{ccc}
% \includegraphics[width=51mm]{flow-8689} & \includegraphics[width=51mm]{flow-8133259} & \includegraphics[width=51mm]{flow-201} \\
% (a) & (b) & (c) \\[6pt]
% \includegraphics[width=51mm]{flow-9612} & \includegraphics[width=51mm]{flow-1873} & \includegraphics[width=51mm]{flow-3679999} \\
% (d) & (e) & (f) \\[6pt]
% \end{tabular}
\begin{tabular}{cc}
\small
\includegraphics[width=79mm]{flow-8689} & \includegraphics[width=79mm]{flow-8133259} \\
(a) & (b) \\[6pt]
\includegraphics[width=79mm]{flow-1873} & \includegraphics[width=79mm]{flow-3679999} \\
(c) & (d) \\[6pt]
% \includegraphics[width=79mm]{flow-201} & \includegraphics[width=79mm]{flow-9612} \\
% (e) & (f) \\[6pt]
\end{tabular}
\longcaption{Interesting Packet Inter-arrival Patterns by Flow}{
The log-scale y-axis shows inter-arrival delay between packets (in nanoseconds), while the x-axis is packets since start of the flow.}
\label{fig:hp-flows}
\end{figure*}

Figure \ref{fig:hp-flows} showcases four hand-selected flows extracted from the 2012 Sanjose CAIDA dataset\footnote{CAIDA Equinix Sanjose January 2012 pcap trace: equinix-sanjose.20120119.}
in order to showcase a few representative multi-modal patterns.
% Example flows are that can be January 2012 CAIDA Equinix Sanjose dataset.
% Four hand-picked examples of flows within CAIDA Equinix Sanjose 2012 January dataset
These plots should be interpreted not strictly as a linear time-series, but similar to a waterfall plot drawn across the x-axis, where the y-axis is a probability density of delays between packets.


Clusters of packet inter-arrival below the approximate transport layer Round Trip Time (RTT)\footnote{RTT is a measure of round-trip latency between two end-hosts -- commonly on the order of 10ms to 100ms for Internet traffic.}
can be considered packet bursts.
Similarly, inter-arrival delays around RTT can be roughly attributed to short-term transport-layer behavior.
Finally, inter-arrival delays far exceeding RTT processing are likely attributable strictly to application level behavior, with an upper bound on flow keep-alive\footnote{Keep-Alive is a common transport-layer timeout concept, primarily used to ensure a dormant flow remains tracked in stateful Flow Tables -- usually on the order of seconds.}
delays.


While packet inter-arrival are inherently noisy, these flows appear to exhibit potential predictable, modal, almost cyclic patterns.
We theorize that the large discrete shifts in packet inter-arrival delays are driven by end-host application behavior and are not simply transients in network conditions.
In the context of cache management, these shifts in application behavior most notably impact packet burst duration and inter-frequency.
Here we aim to explore whether there are cacheable patterns above what the canonical LRU replacement policy is able to identify.
% While further study is needed to truly explain and categorize inter-arrival patterns and their dynamics when competing for cache resources.

% Maybe expand on types of network application patterns?  Streaming, File Transfer, Interactive, Web, ...?
% Networking traffic is often much more than simple



\subsection{Stack-based Algorithms} \label{sec:hp-stack}
Cache management algorithms that maintain ranked order for replacement or insertion are formally referred to as stack-based algorithms.
The Least Recently Used (LRU) algorithm intuitively maintains a replacement stack ordered by last access time.
Specifically, LRU is analgous to Belady's MIN reversed in time -- ranking past instead of future accesses.
Ultimately, LRU is effective when past history leads to a good prediction of the future.

% LRU works well when the cache size is able to capture the working-set; thus past access tends to be representative of future accesses.
% Similarly LRU's effectiveness degrades as the working set grows past the cache size.

% Additionally, flows compete for cache resources adding complexity and noise to cache management analogous to multi-process workloads in processor microarchitecture.

% However, LRU is known to struggle with streaming accesses.
% \footnote{Streaming accesses have little reuse, lowering cache efficiency.}
% Similarly, network flows do not consume equal proportions of bandwidth, nor do they arrive in a purely random process.

% Since LRU only considers the duration since last access, it fails to properly rank future access probability when flows shift between modes of operation.
% bursty and dormant?

% While LRU tends to generally perform well, its simplicity also makes it susceptible to disruption as cache resources are stressed.

%In the context of flow caches, cache streaming patterns would be analogous to flows with low...
%Unfriendly flows in this context is defined as flows that have an average 1/pps \ge time-decay of the cache.

% Primary observation being that LRU works poorly when low recurrance flows are interspersed with high locality flows.
% You can point out that we think similar things are going on with network traffic but we can show that these don't work particularly well.
% Then you want to discuss LIP/DIP/etc as separate, where they are trying to differentiate those items with some recurrance from those with none in different ways.

% Cache management heuristics either explicitly or implicitly 
% LRU implicity inserts new items at the top of the LRU stack

LRU assumes reuse is always likely, inserting all new items in the most-recent position.
Adaptive insertion policies such as Dual Insertion Policy (DIP) \cite{patt-joel-dip}, allow insertion into either the top or bottom of the LRU recency stack.
DIP is similar to bypassing the cache entirely, but does grant the demoted insertion a chance to become promoted.
Adjusting the promotion/demotion logic of LRU can improve cache efficiency in the context of unequal probability of reuse \cite{jiminez-lru-promotion}.

Replacement policies based on reference counts have proven useful as a means to capture temporal patterns.
Cache Bursts \cite{doug-cachebursts} introduced both RefCount and BurstCount as mechanisms estimate reuse predictions from cache entry hit counters.
Reference interval counting mechanisms continue to be researched and improved, leading to Re-Reference Interval Prediction (RRIP) \cite{joel-rrip} and Signature-based Hit Predictor (SHiP) \cite{joel-ship}.


% TODO:
% Its a bit of shift to start talking about BP here, maybe this should be a new sub-sub section on ML techniques in hardware prediction?
Branch prediction research has long been combining multiple information sources, leading to mechanisms to combine or prioritize multiple predictors.
The TAGE predictor is similarly able to combine multiple predictions in a ranking mechanism to select a most likely accurate prediction \cite{seznec-tage2}.
While the Hashed Perceptron mechanism has been steadily gaining momentum as a robust means to consider multiple potentially indicative features together as a whole \cite{jiminez-hp-bp, tarjan-hp-gshare}.

The Hashed Perceptron technique originated in branch prediction, but has been successfully applied to cache management \cite{samira-hp-sampling, teran-reuse-prediction,  chirp-reuse, teran-multiperspective}.
Recent research has also leverage the Hashed Perceptron structure as a filtering mechanism to improve prefetching quality \cite{eshan-hp-prefetch}.
Similar efforts towards prefetching filtering were also accomplished using Bloom Filters \cite{i-spy}.

Several research efforts have applied offline deep learning techniques towards cache replacement \cite{lin-deep-replacement}.
Similarly, Hawkeye \cite{lin-belady-hawkeye} leveraging a time-delayed belady's min algorithm as an online replacement prediction feedback mechanism.



\subsubsection{Preliminary Exploration} \label{sec:hp-failures}
In processor microarchitecture, access patterns are constantly shifting, depending on program behavior.
Similarly in networking, flows also exhibit modes of operation depending on the protocol transport layer as well as end-host program phases.
In the context of a flow table cache replacement policy, LRU does a decent job capturing short-term packet bursts.
 % as long as their inter-arrival delays are smaller than the cache working set.
However, LRU's ranking can also be polluted by dormant, low-bandwidth flows competing for cache resources.
LRU has no way to differentiate reuse probability, treating all flows as equally likely.

The insertion policy is especially critical to flow table cache management due to the short lifetime of most flows.
Most flows are short lived with the majority of bandwidth attributed to a small subset of flows \cite{mchale-bloom}.
However, it is particularly challenging to predict which flows will be short lived early in the flow life-cycle.

Inspired by prior works in CacheBursts \cite{doug-cachebursts} and SHiP \cite{joel-ship}, cache entry hit counters seemed well suited as a means to track packet bursts.
However, early attempts at leveraging CacheBursts and SHiP directly as cache management strategies resulted in performance degradation compared to baseline LRU implementations when applied to flow table cache management.
That said, CacheBursts ended up being a notably informative feature component in our proposed final design.

Our single-perspective cache management approaches were not able to outperform LRU replacement when applied to managing flow tables.
Packet arrival variability inherent in networking adds significant noise to simple pattern predictors such that simple predictor tables alone could not outperform a baseline LRU implementation.
It became evident that a more robust pattern correlation mechanism is needed to rank reuse probability amongst noisy inter-arrival patterns.
% We found that singular approaches heuristic approaches were not sufficient to cope with changing network conditions.

% Further analysis of cache efficiency is provided in Section \ref{sec:hp-efficiency}.



\subsection{Hashed Perceptron Binary Classifier} \label{sec:hp-perceptron}
% You want to frame this part with a discussion about how the key problem is how to classify differnt flows between high and low locality.
% While DIP/LIP/etc don't work well for network traffic, there has been prior work in the processor domain to use a true ML classifier for the job, a Hashed perceptron.  Then the rest of this flows.

The Hashed Perceptron binary classifier has been successfully used in processor microarchitecture as an approach to improve cache management heuristics.
While research on how to integrate and apply this prediction technique has extended over a decade, the technique is now being shipped in modern processors in recent years.

%%%%%%%%% Talk about perceptron model...?
Much like modern machine learning approaches, the Hashed Perceptron improves overall reuse prediction quality by combining multiple predictive features into a singular weighted prediction.
While conceptually similar to perceptrons in a single-layer neural network, the Hashed Perceptron has the significant advantage of being efficient to implement in both hardware and software.
The Hashed Perceptron is also paired with an adaptive training technique to adjust to changing run-time behavior.

Differing from a traditional Perceptron model which scale analog values, requiring integral meaning for each perceptron input.
The Hashed Perceptron is able to map disjoint binary inputs to a corresponding correlation using the feature's table.
The correlation output can be interpreted as an integral value, expressing a historical correlation of a particular feature to the inference question at hand.
During inference, combining multiple features' independent correlations result in a strengthened overall prediction.

% In general, the Hashed Perceptron is well suited to approximations of binary classification.
The processor microarchitecture community has demonstrated the Hashed Perceptron is well suited for reuse prediction, performing especially well in noisy multicore cache hierarchies.
This chapter outlines our exploration into adapting the Hashed Perceptron mechanism to flow table cache management.

% By correlating input Features with observed cacheline reuse, thisHashed Perceptron provides a mapping from observable flow and cache pressure to a relative ranking of expected cache utility.
% The Features, selected at design-time, are ideally chosen to offer unique perspectives to flow behavior.

Our early exploration discovered that relying on any single feature is fragile, especially when applied to network flow table cache management.
Traditional single-feature approaches failed to surpass the consistent performance of LRU when applied to network caching.
The variety of traffic patterns encountered in network cache management demands a general approach to consistently approximate a good working set.

Caching will continue to be a fundamental component of network data planes as a means to amortize costly control path decisions.
The trend in networking to support programmability of generic network functions increases control path complexity.
Advances in cache management strategies leveraged in modern processor microarchitecture are absent in the networking domain.
Clearly there is a gap between Belady and LRU, can we do better?




==> hp-mcc.tex <==


\section{Matthew's Correlation Coefficient} \label{appendix:mcc}
This appendix aims simplify the interpretation of MCC by Equation \ref{eq:mcc-2}.
Pearson's Correlation Coefficient is defined in Equation \ref{eq:corr-1}.
\begin{equation} \label{eq:corr-1}
PCC = corr(X,Y) = \frac{cov(X,Y)}{\sigma_X \sigma_Y}
\end{equation}

Equation \ref{eq:corr-2} is rewritten with respect to covariance and variance:
\begin{equation} \label{eq:corr-2}
corr(X,Y) = \frac{cov(X,Y)}{\sqrt{var(X)} \sqrt{var(Y)}}
\end{equation}

Equation \ref{eq:corr-2} is further rewritten in terms of expected value:
\begin{equation} \label{eq:corr-3}
corr(X,Y) = \frac{E[(X - \mu_X)(Y - \mu_Y)]}{\sqrt{E(X^2)-E(X)^2} \sqrt{E(Y^2)-E(Y)^2}}
\end{equation}

Matthew discovered restricting Pearson's Correlation Coefficient to binary classes allows for simplification.
After manipulation, and reduction, MCC is commonly represented as seen in Equation \ref{eq:mcc}.
\begin{equation} \label{eq:mcc}
MCC = \frac{TP*TN - FP*FN}{\sqrt{(TP+FP)(TP+FN)(TN+FP)(TN+FN)}}
\end{equation}

By correlating the predictions against actual, MCC balances the predictor accuracy across both classes.
Matthew's Correlation Coefficient can be interpreted as bisections of the confusion matrix:
\begin{equation} \label{eq:mcc-2}
MCC = \frac{correct(X,Y) - incorrect(X,Y)}{\sqrt{actual(X,Y) * predicted(X,Y)}}
\end{equation}

Where the numerator contains the \emph{difference of products} between the correct diagonal (Equation \ref{eq:mcc-correct}) and vs the incorrect diagonal (Equation \ref{eq:mcc-incorrect}).
\begin{equation} \label{eq:mcc-correct}
correct(X,Y) = TP*TN
\end{equation}

\begin{equation} \label{eq:mcc-incorrect}
incorrect(X,Y) = FP*FN
\end{equation}

Normalized by a denominator consisting of \emph{product of sums} across actual ground truth rows (Equation \ref{eq:mcc-actual}) vs prediction columns (Equation \ref{eq:mcc-predicted}).
\begin{equation} \label{eq:mcc-actual}
actual(X,Y) = (TP+FN)(TN+FP)
\end{equation}

\begin{equation} \label{eq:mcc-predicted}
predicted(X,Y) = (TP+FP)(TN+FN)
\end{equation}


==> hp-results.tex <==




\section{Analysis} \label{sec:hp-analysis}
The primary evaluation goal of this work is to assess the viability of applying the Hashed Perceptron correlation mechanism to stateful flow table cache management.
Contrasted with the cache optimality limit study in Section \ref{sec:hp-opt}, this feasibility study provides insight into practically capturable locality.

% Section \ref{sec:hp-methodology} describes the cache simulation and evaluation methodology.
% We first evaluate several competing feature ranking mechanisms in Section \ref{sec:hp-fsa}.
% Second, we evaluate the robustness of the best performing features across different datasets, cache pressures, and design parameters in Section \ref{sec:hp-performance}.
% In Section \ref{sec:hp-efficiency} we try to gain intuition of cache management behavior by analyzing differences in cache efficiency between baseline LRU, Belady's MIN, and our flow correlator mechanism.
% Finally Section \ref{sec:hp-roles} recaps some of the dynamics between the features chosen for the flow correlation mechanism.

% Section \ref{sec:hp-fsa} walks through feature selection, feature ranking, and iterative information gain.
% Section \ref{sec:hp-performance} compares test-set and validation-set improvements across th.
% Section \ref{sec:hp-efficiency} provides some insight into cache entry behavior through cache efficiency.


\subsection{Methodology} \label{sec:hp-methodology}
%Describe simulator, test data sets, performance assumptions, etc.
The simulator developed for this study allowed for quick exploration of cache management strategies in the context of stateful network flow tables.
This work focused on cache hit-rate as the primary performance metric with the expectation that cache hit-rate translates directly into improved throughput and ultimately cache efficiency.
While this cache hit-rate simulation does not model the latency intricacies incurred by cache misses as well as flow table management, it does showcase relative prediction accuracy of competing cache management algorithms.
Focusing on cache hit-rate simulation for the viability study allows for quick design iteration.



\subsubsection{Network Traffic Datasets}
It is tempting to leverage synthesized network traffic based on statistical models of packet arrival behavior \cite{traffic-gen, traffic-gen-validation}.
However, the random packet inter-arrival assumptions of these models would both hinder the cache management algorithm as well as introduce uncertainly around the accuracy of the synthesized traces.
While these models can quite accurately resemble real inter-arrival flow behavior, actual packet arrival behavior is inherently complex and beyond our confidence to model.
This viability study hinges on having representative datasets of network traffic to validate the premise of capturable temporal locality through more advanced cache management techniques.
% Utilizing a realistic input dataset, representative of network traffic is crucial to this viability study.

For this study, we chose to leverage network packet capture (PCAP) traces rather than synthetic traffic in order to preserve temporal inter-arrival patterns theorized to be present in Section \ref{sec:hp-patterns}.
% This work instead aims to test the viability of hashed perceptron based flow table cache management.
CAIDA's offers passive PCAP traces within their Equinix internet exchange\footnote{Internet Exchange Points (IXPs) are crucial infrastructural components of the Internet where network operators (peers) exchange traffic.}
data centers. 
We leveraged PCAP traces from CAIDA Equinix Sanjose, Chicago, and NYC datasets spanning 2012 to 2018 \cite{caida-cache}.
% CAIDA Equinix PCAP traces were selected because of their deserve and representative subset of internet traffic.
Traffic flowing through these exchange points should contain a representative sampling network traffic commonly found on the Internet.
CAIDA's Equinix datasets were chosen primarily because of the availability and diversity of the traffic provided and available to researchers.

\begin{table}[ht]
\small
\centering
\singlespacing
\begin{tabular}{|r|l|}
\hline
\textbf{CAIDA Dataset} & 
    Equinix Sanjose January 2012 \\ \hline
\textbf{Interface} &
    10 Gbps link (6 Gbps average, bi-directional) \\ \hline
\textbf{Packet Rate} & 
    1M / second \\ \hline
\textbf{New Flows} & 
    30k / second \\ \hline
\textbf{Active Flows} & 
    300k over 4-second window \\ \hline
\textbf{Trace Length} & 5 minutes \\ \hline
\end{tabular}
\caption{Sample of CAIDA Packet Arrival Statistics}
\label{tbl:hp-caida-stats}
\end{table}

The CAIDA Equinix PCAP traces utilized for this study are captured on 10 Gbps links and taken over one hour intervals, split into 1 minute files.
Table \ref{tbl:hp-caida-stats} provide a summary of packet arrival and flow turnover statistics.
The CAIDA PCAP files contain pseudo-anonymized network layer IPv4 addresses, preserving subnets while anonymizing exact addressing.
Because of the inherent complexities involved, we believe actual traces of representative network traffic to be crucial in exploring the viability of network flow table cache management.



\subsubsection{Cache Simulation}
The simulator models a single inline device maintaining a stateful flow table such a firewall.
Maintaining this stateful flow table is the critical-path for achievable throughput.
Caching techniques are leveraged to improve device throughput; this study focuses on improving the approach of cache management by borrowing techniques developed within the the computer microarchitecture community.

\begin{table}[ht]
\small
\centering
\singlespacing
\begin{tabular}{|r|l|}
\hline
\textbf{Flow Cache Entries} & 
    4k flow entries \\ \hline
\textbf{Cache Associativity} &
    8-way \\ \hline
\textbf{Feature Tables} & \makecell[l]{
    5 features, each 64k entries \\
    5-bit saturating counters} \\ \hline
\textbf{Feedback History} & 
    8 predictions / associative-set \\ \hline
\textbf{Feature Selection Dataset} & 
    CAIDA Equinix Sanjose January 2012 \\ \hline
\textbf{Validation Datasets} & \makecell[l]{
    CAIDA Equinix Sanjose March 2012 \\
    CAIDA Equinix Chicago March 2014 \\
    CAIDA Equinix Chicago March 2016 \\
    CAIDA Equinix NYC March 2018} \\ \hline
\end{tabular}
\caption{Hashed Perceptron Cache Simulation Parameters}
\label{tbl:hp-cache-simulation}
\end{table}

Table \ref{tbl:hp-cache-simulation} summarizes the cache simulation parameters as well as feature selection and validation datasets.
The simulator replays PCAP files, preserving relative arrival order to maintain packet inter-arrival patterns.
The packet headers are parsed, stateful flow identifiers maintained throughout the simulation to track and evaluate cache management algorithm's relative performance.
%Since flow identifiers are implicit, a forgiving heuristic is required to track flow state from single directional flow data.
In addition to cache hit-rates, the simulator gathers evaluation metrics helpful to gain insight during early design exploration of the \emph{Flow Correlator} cache management mechanism described in Section \ref{sec:hp-hp-design}.

% TODO:
% Have a table of the number cache of entries for the different experiements and other parameters explored


We first provide insight into our feature exploration, evaluating several competing feature ranking mechanisms in Section \ref{sec:hp-exploration}.
Second, we evaluate the robustness of the final selected features across datasets in Section \ref{sec:hp-performance}.
In Section \ref{sec:hp-efficiency} we infer changes in cache entry lifetime by analyzing cache efficiency.
Finally, Section \ref{sec:hp-roles} recaps some of the dynamics between the chosen features in the context of bypass and reuse cache management predictions.
% Appendix , provides insight into sensitivity to cache pressures and design parameters.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Feature Exploration} \label{sec:hp-exploration}
While performance estimation is the ultimate goal of any architectural design-space exploration, quickly ranking useful features early in the design process is immensely valuable.
Feature design, ranking, and selection is a time-consuming component of design exploration -- adding yet another dimension to an already complex optimization problem.
% Feature selection and design-space optimization are immense fields of research which can be applied here.
% This section analyzes the effectiveness of our automated feature ranking highlighted in Section \ref{sec:hp-selection} as well our hand-picked features.

Since nearly all of the features explored in Table \ref{tbl:hp-all-features} perform poorly in isolation, it is crucial to compare feature performance as a system.
Further, it becomes non-trivial to select the best combinations of feature components as candidate combinations inherently share mutual information.
% for any independent feature ranking mechanism to select amongst feature combinations
Therefore, there is a need for a reliable ranking mechanism that allows the architect to identify top performing feature combinations early in the design phase.
% The ability to rank features after a single simulation run O(1) opposed to O(N) required by the differential analysis.
% While crucial for the analysis of the feature ranking mechanisms described in this section, differential analysis is computationally expensive, requiring O(N) runs just for feature comparison.

The two competing feature ranking techniques analyzed in this section are Matthews Correlation Coefficient (MCC) and Total Influence (INF).
Randomly ordered features (RND) were also included to gauge the effectiveness of the mechanisms in context.
Finally, we describe a differential analysis technique developed in this work to trim mutual information, resulting in the final feature ranking.

% Sweep of features explored during design-time feature selection and hit-rate improvement analysis.


% discuss which technique best selects top performing features.
% \begin{itemize}
% \item[p *] Show difference in feature performance depending on cache operating conditions (comfortable, stressed, congested).
% \item Performance approaches baseline (LRU) when system is conservative.
% \end{itemize}

% \subsubsection{Feature Extraction}
% comment in design that this was not automated?..


\subsubsection{Feature Design} \label{sec:hp-feature-design}
% During the feature design phase of this work
\emph{Influence} was discovered out of a desire for feedback during feature design.
% With finite \emph{pure} and \emph{pattern} feature components,
In particular, hints at strengths and weaknesses of competing features help identify successful mixing strategies early in the design exploration.
% , leading to further improvements in future combinations.
The intuition behind Influence centers around interpreting the feature's correlation output (weight) as a confidence.
Influence then contrasts these contribution confidences against the overall correctness of the system, grouped by prediction type (Reuse or Bypass).
% Tracking the confidence for each prediction across the confusion matrix as shown in Table \ref{tab:hp-influence-matrix} 

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{2012-sanjose_feature-reuse_rank-mcc}
\caption{Feature Influence on Reuse Predictions}
\label{fig:hp-reuse-mcc}
\end{figure}

Figure \ref{fig:hp-reuse-mcc} provides insight into feature contributions towards flow entry reuse predictions, relative to MCC's balanced prediction accuracy.
Per-feature MCC and Influence metrics are tracked across all candidates in a single Hashed Perceptron \emph{Flow Correlation} simulation.
Features are sorted in decreasing MCC order with the corresponding \emph{Correct Influence} and \emph{Incorrect Influence} presented for relative comparison.
% The y-axis of this plot can be interpreted as the average contributed confidence (weights) of each competing feature.
% NOTE: elaborate at the difference between Correct and Incorrect Influence?


The first entry, \emph{System}, represents the overall flow entry reuse prediction exhibiting a notable improvement in MCC compared to any individual feature.
% only relative accuracy being unimportant in this context.
% Contrasting \emph{Correct Influence} against \emph{Incorrect Influence} for each feature 
% Influence provides unique insight into 
The contributions towards correct predictions (\emph{Correct Influence}) as well as contributions towards incorrect predictions (\emph{Incorrect Influence}) represent a feature's influence over the predictor.
The magnitude represents confidence while the sign represents a positive (or negative) influence on predictor outcomes.
 % with respect to \emph{System} predictions.
% The purpose of Feature Influence is to bisect the relative MCC metric by each feature's contributions towards correct and incorrect system decisions.

Interestingly, features exhibiting high confidence towards correct predictions tend to also be accompanied by overconfidence towards incorrect predictions.
Overconfidence can be tolerated when coupled with a high prediction accuracy (MCC); however, there is a strong preference for features that provide value while also minimally contributing to mispredictions as represented by \emph{Incorrect Influence}.
% A few notable exceptions center around combinations of the IP frame length (Pure Feature $f_{11}$) as well as global correlation of packet sequence ($f_{10}$) to reuse probability.
% this would be a really good time to look at the weight map for F10...


%%%%%%%%%%%%%%%%%
% You need a paragraph or 2 to describe how, the bypass figure, is different from the other figure.


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{2012-sanjose_feature-bypass_rank-mcc} 
\caption{Feature Influence on Bypass Predictions}
\label{fig:hp-bypass-mcc}
\end{figure}

% The bypass flow entry predictions must triage 
Figure \ref{fig:hp-bypass-mcc} provides insight into feature contributions towards flow entry bypass predictions relative to MCC.
It is intuitive that features have strengths towards either Bypass or Reuse predictions.
Unlike reuse flow entry predictions, bypass predictions inherently lack some of the temporal indicators tracked in cached flow table entries.

Bypass and Reuse predictions both aim to predict flow entry reuse within the approximation of the useful cache working set.
However, they are distinct predictions as reuse probability of a cached and uncached flow table entry are not necessarily equivalent.
Bypass predictions occur not only at the start of new flows, but also on transitions from \emph{Dormant} to \emph{Active} for already established flows.
Reuse predictions aim to identify \emph{Active} connections amongst established flows, triggering early eviction if predicted to transition from \emph{Active} to \emph{Dormant}.


% The hashed perceptron mechanism relies on regulated feature confidence, enabling the consensus to reach a more informed prediction.
% Features that provide insight while remaining constrained when incorrect are notable valuable.


% The accumulated contributions are scaled by the number of respective predictions such that the plotted value can be interpreted similar to an average confidence relative to the range of weights.

% Correct System Decision
% + : Contribution towards correct consensus
% - : Protested against ultimately correct decision

% Incorrect System Decision
% + : Protested against incorrect decision, but ultimately overuled
% - : Contributed towards incorrect consensus

% Referring back to Section \ref{sec:hp-influence} for definitions of the Influence metrics.
% % \emph{Correct Influence} is interpreted as accumulated contributions towards correct system decisions.
% \emph{Correct Influence} is calculated using Equation \ref{eq:f-correct-inf} for each feature with respect to correct system decisions.
% Similarly, \emph{Incorrect Influence} is calculated using Equation \ref{eq:f-incorrect-inf} with respect to incorrect system decisions.



% Most Burst Count and Reference Count combinations seem moderately informative with only hints of utility provided by improved \emph{Incorrect Influence}.
% move/discuss why in final feature choice section.


% It is notable value is provided to the system when allowed to decouple from an assumption of global reuse burst patterns across all flows.
% However, it is also interesting to note that there appears to be particular value mixing burst patterns with IP frame length ($f_{27}$).



% Figure \ref{fig:hp-reuse-mcc} contrasts Influence components for Reuse Predictions while Figure \ref{fig:hp-bypass-mcc} contracts bypass...

% While Bypass and Reuse are conceptually distinct predictions, they share correlation tables in this study.

% TODO: Finish this thought...
% Features with largely negative \emph{Incorrect Influence} with a high MCC exhibit more overconfidence, contributing towards incorrect decisions.
% Conversely, Features with relatively less \emph{Incorrect Influence} 

% \begin{figure*} [ht]
% \begin{tabular}{cc}
% \includegraphics[width=85mm]{2012-sanjose_feature-reuse_rank-mcc} & \includegraphics[width=85mm]{2012-sanjose_feature-bypass_rank-mcc} \\
% Reuse & Bypass \\[6pt]
% \end{tabular}
% \caption{Feature Ranking sorted by MCC}
% \end{figure*}

% \subsubsection{Feature Selection: Bypass}
% certainly insightful as a viewport into feature's role in the system (see feature roles section)


Burst Count and Reference Count (Pure features $f_{14}$ and $f_{15}$) exhibit a perplexing anti-correlation as seen by both MCC and Influence.
It is notable that Burst and Reference Count rely on unrolled and allowed to decouple from global patterns.
% Influence provides insight that BurstCount and RefCount (as a global counter) behave like a single entry correlator (NULL control feature)
Intuitively, it makes sense that temporal patterns need to be grouped (unrolled) in some way to enable correlations.
% The Flow Correlator mechanism seems to prefer temporal feature unrolling somewhere between global and fully specified flowID.
During feature design, Influence enabled insight into how each feature fell into natural cache management roles.


% Features useful for bypass
% Features useful for early eviction (resuse estimation)

% reject oriented features
% accept oriented features
% bias implies unbalanced, we saw features naturally fit 

% \begin{itemize} \label{f-roles}
% \item Cache management role: Bypass vs Reuse
% \item Feature Role: Pessimistic vs Optimistic
% \end{itemize}


\subsubsection{Feature Ranking} \label{sec:hp-ranking}

\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{2012-sanjose_speedup-rank-order-4k} 
\longcaption{Initial Feature Ranking}{
Hit-rate improvement over baseline LRU comparing MCC-4k below bars in yellow to INF-4k above in blue.}
\label{fig:hp-rank-initial}
\end{figure}

Figure \ref{fig:hp-rank-initial} shows the relative hit-rate improvement over LRU as baseline.
\emph{Total Influence} as defined in \ref{eq:f-total-inf} was used for INF-4k's ranking.
The plot is generated by incrementally including features in ranked order using Algorithm \ref{alg:hp-sweep}.
This \emph{sweep} plot shows the incremental gain in hit-rate by including additional features as a useful means to compare feature rankings.
Spanning from a single feature (left) to all features (right), diminishing returns can be easily identified.
% difficult to describe how plot is generated....
% 1) inital ranking for MCC and INF
% 2) non-obvious combination of Bypass and Reuse
% 3) hit-rate simulation runs from f1 -> fN to validate if ranking order maps to gain in perforamnce metric
% 4) note that earlier features inherently look better (less information already provided)
% 5) lead to insights covered in next section....

% $f_{1}


% Since Influence weights
% Interpreting MCC as a balanced accuracy isn't quite sufficient..
% It is interesting to note that INF has a slight preference for features exhibiting n
% This highlights how Influence is useful, especially during feature selection.

% It is interesting to highlight a few dependencies between MCC and INF.

% One of the inherent complications of ranking features individually
% shared information
 % that contribute towards a larger system predictor 

Both MCC and INF provide a relatively similar ranking, with a few notable differences.
In particular MCC's top choice, $f_{4}$ consists of just TCP flags is unable to stand alone.
INF's top choice, $f_{6}$, consists of a mix of Port, Protocol, and TCP/IP flags, covering $f_{4}$.
As a single-table predictor, INF's $f_{6}$ manages to provide a modest 2\% hit-rate improvement over baseline LRU, while MCC's $f_{4}$ actually degrades hit-rate.
Ultimately MCC provides a better all-rounded ranking; however, INF does identify a few notably valuable features before MCC.

% \subsubsection{Feature Ranking: Control}
To help put into perspective the utility of MCC as a feature ranking mechanism, we compare against four randomized rankings.
As expected, Figure \ref{fig:hp-rank-random} showcases the stunted performance of random rankings amongst features with significant permutation overlap.
There are a few notable observations that highlight the behavior of a Hashed Perceptron based predictor.


\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{2012-sanjose_speedup-rank-order-4k-random}
\caption{Random Feature Ranking}
% RND1: \\
% RND2: \\
% RND3: \\
% RND4: 
\label{fig:hp-rank-random}
\end{figure}


The first notable observation is that predictor effectiveness under-performs baseline LRU until the third randomly selected feature is added.
The situation flips with the third random selection able to surpass baseline; achieving half the potential hit-rate improvement by the fourth random selection.
% Secondly, it is interesting to note that over half the gain is achievable by only five random features.

As expected, there is significant shared information across the features in Table \ref{tbl:hp-all-features} due to feature permutation similarity.
The goal of the ranking algorithm is to identify the best combinations in order to hasten designer iteration.
It is clear that MCC and INF are both able to identify a better initial ranking than random selections.
However, MCC and INF are both unable to account for shared information, looking only at the feature's own track record in isolation.


\subsubsection{Iterative Information Gain} \label{sec:hp-rank-ig}
% \subsubsection{Feature Ranking: Differential Gain}
% Naively selecting just the top five features from either MCC or INF results in .
Relying on the designer to select the best choice is untenable as system complexity grows.
Ultimately we need a method to rank features by incremental value contributed to the system.
Inspired by information gain decision tree learning algorithms, we outline our approach to both measure a feature's actual contribution to the system as well as take into account mutual information between features.

Our iterative information gain method outlined in Section \ref{sec:hp-information-gain} improves a MCC ranking by differential analysis sweep.
The feature sweep analysis plot is differential analysis, where hit-rate is plotted as features are incrementally added until all features are included.
Figure \ref{fig:hp-rank-differential} shows the incremental change in hit-rate as features are incrementally added to the predictor in MCC-4k rank-order.


\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{2012-sanjose_speedup-rank-order-4k-differential}
\longcaption{Differential Improvement}{
Per-feature hit-rate differential gain (adjacent difference) of MCC-4k.}
\label{fig:hp-rank-differential}
\end{figure}

Figure \ref{fig:hp-rank-differential} shows the change in hit-rate as features are added to the predictor from left to right.
While early features are likely to bring a larger gain, the goal is to minimize shared information between features.


\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{2012-sanjose_speedup-rank-order-4k-IGn} 
\caption{Iterative Information Gain Ranking Improvement}
% {Plotting the rank improvement for the first ten features.}
\label{fig:hp-rank-ig}
\end{figure}

Figure \ref{fig:hp-rank-ig} shows the iterative improvement from the initial \emph{MCC-4k} ranking through three iterations of differential information gain.
To improve readability, this figure just showcases the hit-rate improvement for the first ten features.
\emph{IG\textsubscript{1}-4k} through \emph{IG\textsubscript{3}-4k} represent the improvement in ranking through each differential Information Gain (IG) iteration.
% \emph{IG\textsubscript{3}-4k} was chosen as final ranking (\emph{IG-4k}).

The first notable adjustment made in the first pass (IG\textsubscript{1}) is identifying that $f_{6}$ covers $f_{4}$ entirely and translates to a hit-rate improvement as the first feature, despite $f_{4}$ achieving a marginally higher prediction accuracy as inferred by MCC.

It is also notable that $f_{10}$ and $f_{18}$ were both overlooked by MCC and INF implying a relatively low prediction accuracy.
However, both propagated to the top five ranking in the subsequent two iterations (IG\textsubscript{2} and IG\textsubscript{3}).
This differential information gain analysis identified that $f_{10}$ and $f_{18}$ provided notable value to the system, despite the lower prediction accuracy.

The final notable adjustments were marginal, preferring to unroll across upper IP addresses rather than middle or lower variants ($f_{18}$ and $f_{21}$).

This iterative information gain technique is best fit to trim shared information from an already decent ranking.
% The technique's iterative requirement is due to the complex dynamics of 
While not showed here, attempts to iterate from a random feature selection using just the iterative information gain technique was computationally prohibitive.

We found Influence to be a particularly useful during feature creation, MCC best suited for initial feature ranking, and differential information gain notably helpful to narrow in on the most informative features.
Automating feature selection, even if imperfect, allows the system designer to focus on feature creation -- in particular introducing novel feature combinations and information sources.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Cache Hit-Rate} \label{sec:hp-performance}
\subsection{Improvement Validation} \label{sec:hp-performance}
% Analysis of steady-state performance of hashed perceptron reuse predictor.



% \subsubsection{Attainable Hit-Rate Improvement}
% intend to show how much of improvement is capturable with just topN features.
% show how each feature behaves and contributes to an overall better system performance...


% \subsubsection{Final Feature Selection} \label{sec:hp-final-features}
% The best feature ranking from Section \ref{}

\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{2012-sanjose_speedup-rank-order-4k-comp} 
\caption{Final Feature Ranking Comparison}
\label{fig:hp-rank}
\end{figure}

Figure \ref{fig:hp-rank} recaps the ranking improvement on the training dataset.
Diminishing returns in achievable hit-rate improvements started to occur roughly between four and seven features.
For validation, we decided to select the five best features from each ranking.


% A designer must trade-off available hardware resources, number of features, feature table size, as well as hashed perceptron feedback queue depths.
% The scope of this analysis is limited to validating


\begin{table}[H]
% remove extra \newline incured by wrapped tables (thesis office fix)
\vspace{-\baselineskip}
\small
\centering
\singlespacing
\begin{tabular}{cll}
% \begin{tabular}{cllp{0.35\linewidth}}
\textbf{$f_{\#}$} & \textbf{Feature Type} & \textbf{Feature Components} \\
6  & Pure Mix & $f_{TCP}\!\ll\!7 \wedge ipProto \wedge min(srcPort, dstPort)$ \\
27 & Pure + Pattern & $\{ipLength, \lceil burstCount \rceil_8 \}$ \\
21 & Pure + Pattern & $ipLength \wedge (ipv4Dst \wedge ipv4Src)[31\!\colon\!16]$ \\
18 & Pure + Pattern & $\{\lceil refCount \rceil_8, \lceil burstCount \rceil_8\} \wedge (ipv4Dst \wedge ipv4Src)[31\!\colon\!16]$ \\
10 & Pattern & $\lceil flowPackets \rceil_{16}$
\end{tabular}
\longcaption{Selected Features (IG\textsubscript{3}-4k)}{
Optimized on flow cache with 4k entries, 8-way set associativity using the CAIDA Equinix Sanjose January 2012 dataset (equinix-sanjose.20120119) during feature selection and ranking.}
\label{tbl:hp-selected-features}
\end{table}


% The final features used
Table \ref{tbl:hp-selected-features} list the top five features in ranked order of improved system value after the third iteration of differential information gain (IG\textsubscript{3}-4k).
% Listed in relative order of improved system value after the third information gain iteration (IG-4k) as shown in Figure \ref{fig:hp-rank}.
It is interesting to note that all \emph{Pure} information sources were utilized in some form in the final set of features.
While it is not surprising that protocol and TCP/IP flags proved to be a naturally useful reuse hints, it is certainly interesting that $f_{6}$ was preferred over the $f_{4}$.
 % or per-flow f
A similarly useful reuse hint comes from deviations in IP frame length.
While both MCC and INF showed high utility of frame length ($f_{11}$) as a \emph{Pure} indicator, IG\textsubscript{3} found significantly higher utility by combining frame length and BurstCount ($f_{27}$).

It appears that both frame length and BurstCount contributed uniquely as a reuse prediction hint, both notably providing additional value being unrolling over upper IP addresses ($f_{18}$ and $f_{21}$).
With IP address combinations seemingly contributing little insight into reuse as \emph{Pure} sources, it is interesting that both frame length and BurstCount found extra utility through unrolling.
Appendix \ref{appendix:selected} provides further insight into selected features' weight distributions alongside the contributing feature components.
% While omitted from this round-up, packet length is the next intuitive inclusion.
% Frame length is often identical to packet length because of implications of fragmentation, there are still many situations where frames do not match.

% Unrolling is simply a conceptual distinction to convey the intent behind spreading correlation potential across a larger .

% Intuitively we suspected upper IP addresses subnets to be a decent way to unroll \emph{Pure} or \emph{Pattern} sources.

% While subtle, it seems unroll preference is upper16


% These  five features as ranked by IG\textsubscript{3} were selected for subsequent validation and compared against MCC and INF.


% TODO: better elaborate chosen features?
% $f_{6}$: Mix IP protocol, TCP flags, and lowest port
% $f_{27}$: Concatenate BurstCount with frame length
% $f_{21}$: Unroll frame length over upper ip
% $f_{18}$: Unroll Burst/RefCount over upper ip 
% $f_{10}$: Packets since start of flow



\subsubsection{Validation Datasets}
While it is clear that there is notable improvement performing IG passes within the training dataset, it is crucial that this process did not over-optimize feature selection.
The training set consisted of five minutes of PCAP, bi-directional from January 2012 taken at CAIDA Sanjose exchange.
The validation set consisted of five minutes of PCAP, bi-directional from March of 2012, 2014, 2016 and 2018 spanning the three available CAIDA exchange locations: Sanjose, Chicago, and NYC.
The validation set will be used to compare the top-five features provided by the MCC-4k, INF-4k, and IG\textsubscript{3}-4k rankings.

% intend to show selected features are adaptable to other CAIDA traces and is not simply overfit to the 2012-sanjose traces.
\begin{figure}[H]
\centering
\includegraphics[width=0.85\linewidth]{2012-sanjose_speedupValidation}
\caption{Improved Hit-Rate Validation}
\label{fig:hp-validation}
\end{figure}

Figure \ref{fig:hp-validation} shows consistent improvement across all validation sets.
Hit-rate improvements ranged between 4\% and just under 8\% over baseline LRU.
The validation datasets showed no degradation from MCC-4k to IG\textsubscript{3}-4k, indicating that iterative Information Gain did not over optimize.
% Furthermore, we observed a comparable (0.5\%) additional hit-rate gain in the March Sanjose dataset, roughly half that (0.25\%), while NYC
However, we suspect IG's greedy optimization requires generality in feature creation -- best suited to remove mutual information rather than select the most robust features.

 % were less sensitive to Information Gain improvements, emphasizing the 

These results attest to the generality of the features chosen, providing value to a generic cache management reuse predictor beyond the original dataset location.
It is certainly notable to demonstrate viability towards a flow table cache management approach which translates beyond the original optimization parameters.
% Since networking is inherently diverse, this is a crucial point of validation showing the viability to 

% Automated feature creation techniques may become more susceptible to over-optimization, requiring more care.

% \subsubsection{Cache Size}
% indend to show the gap between capturable locality and upper limit provided by belady
% show that there are two shelves of capturable locality which map to two fundamental layers of networking: transport and application


% \subsubsection{Set Associativity}
% this one is complicated as Training Queue Depth is intertwined with Associativity
% an override was defined rellatively last-minute, not substantially explored yet


% \subsubsection{Correlation Feedback Queue Depth}
% continueation of previous discussion around associativity and queue depth?


% \subsubsection{Correlation Table Length}
% Feature input range -> 2^n table entries
% there is a RC time-constant sort of dynamic that is affected by correlation table length, sat. counter entries, etc.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cache Efficiency} \label{sec:hp-efficiency}
% \item Flow Inter-arrival: Flow shift between intervals of inter-arrival access patterns: sequential, random, bursty.  (access patterns are in inter-arrival delays, not address strides in processor caches)
% \item Effective Cache behavior: The superposition of all flow behavior within any given time window is defined as the working set.
% \end{itemize}


Tracking the lifecycle of cache entries can be helpful to understand how cache management techniques impact cache behavior.
Figure \ref{fig:hp-entry-life} depicts a cache entry's lifecycle from insertion ($t_0$) to last-access time ($t_L$) and finally the eviction time ($t_E$).

\begin{figure}[H]
\centering
\includegraphics[width=55mm]{cache-lifetime}
\longcaption{Cache Entry Lifecycle}{
$t_0$: insertion time, $t_L$: last-access time, $t_E$: eviction time}
\label{fig:hp-entry-life}
\end{figure}

Equation \ref{eq:f-lt} defines a cache line's \emph{lifetime} as duration between insertion and last access.

\begin{equation}
lifetime = t_L - t_0
\label{eq:f-lt}
\end{equation}

Similarly, \emph{deadtime} is the duration between last access and eviction as defined in Equation \ref{eq:f-dt}.

\begin{equation}
deadtime = t_L - t_E
\label{eq:f-dt}
\end{equation}

Finally, Equation \ref{eq:f-efficiency} defines cache line \emph{efficiency} as the useful \emph{lifetime} over the total time the cache entry was occupied.

\begin{equation}
efficiency = \frac{t_L - t_0}{t_E - t_0}
\label{eq:f-efficiency}
\end{equation}

Tracking the \emph{lifetime}, \emph{deadtime}, and \emph{efficiency} for all cache lines throughout the simulation provides some insight into the relative impact of cache management algorithms on overall caching behavior.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\linewidth]{4k-8_clockTimeLast} 
\caption{Cache Entry Lifetime}
\label{fig:hp-lifetime}
\end{figure}

Figure \ref{fig:hp-lifetime} compares the cache line \emph{lifetime} during a cache simulation over a one minute pcap trace\footnote[1]{CAIDA Equinix Sanjose January 2012 pcap trace: equinix-sanjose.20120119.}.
While the vast majority of flows entries have a short lifetimes in the cache, the \emph{Flow Correlator} Hashed Perceptron cache management technique (hp) more closely resembles Belady's MIN (min).
Holding onto certain bursty flows for a longer duration between pauses potentially reducing entry turn-over.
% It is notable how the hashed perceptron's lifetime resembles MIN -- choosing to keep certain flows cached for a much longer duration than LRU otherwise would.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\linewidth]{4k-8_clockTimeDead} 
\caption{Cache Entry Deadtime}
\label{fig:hp-deadtime}
\end{figure}

Figure \ref{fig:hp-deadtime} shows the corresponding \emph{deadtime}, implying that the hashed perceptron technique simultaneously has both more and less patience.
A significant number of entries are evicted very early (within 10ms), while simultaneously waiting on average twice as long as LRU for others (upwards of 200ms).
This adaptability allows hp to triage flows with low probability of reuse, while simultaneous willing to increasing entry \emph{deadtime} in hopes of also enabling an increase in entry \emph{lifetime}.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\linewidth]{4k-8_clockTimeEfficiency}
\caption{Cache Entry Efficiency}
\label{fig:hp-efficiency}
\end{figure}

% The average cache line efficiency increased from $x\%$ to $y\%$.
Figure \ref{fig:hp-efficiency} outlines how the hashed perceptron approach generally smoothed out cache \emph{efficiency}.
LRU's inherent requirement to wait for demotion from MRU to LRU limits cache efficiency.
Meanwhile, the hashed perceptron technique is a step towards both triaging flows with a low probability of reuse as well as a tendency to hold onto cache entries for a longer duration.

Cache \emph{efficiency} doesn't grant perspective into the quantity of hits over the entry \emph{lifetime}, just that the entry had reuse.
Coupled with an improvement to hit-rate, this cache line efficiency analysis confirms that there is a worthwhile trade-off to holding onto certain flows longer as well as triaging flows early.



% \subsubsection{Estimating Working Set}
% working set estimation.  ratio of concurent flows : cache size?
% 10M flows
% 100M cache insertions
% 290M packets
% 50% hit-rate




\subsection{Feature Roles} \label{sec:hp-roles}
Throughout the feature selection process, we noticed a few noteworthy trends in roles assumed by each feature.
 % in contrast to the system as a whole.
Observed primarily through feature influence described in Section \ref{sec:hp-influence}, features tended to produce a certain prediction bias as measured by average output prediction weight.
% favor either bypass or reuse.
Originally described as a form of optimism, features tended to vote for eviction (pessimistic), while others tended to lean towards reuse (optimistic).
What was observed as a natural feature bias towards a particular outcome, in actually reflects the natural predictive utility of the feature.

Certain features are better indicators of early eviction -- hinting at a flow's transition from \emph{active} to \emph{dormant}.
The temporal pattern feature components ($f_{10}$, $f_{14}$, and $f_{15}$) are clear contributes to bypass role.
Other features are best suited to triage incoming flows during bypass -- hinting at flow transitions from \emph{dormant} to \emph{active}.
Indications of protocol behavior from several pure feature components ($f_{4}$, $f_{6}$, and $f_{11}$) were notable contributions to the reuse role.

These two cache management roles (bypass and reuse) tend to uniquely favor subsets of feature components.
In nearly all cases, we noticed an overall benefit in combining feature components with orthogonal roles.
Additionally, we also noticed that certain orthogonal combinations ($f_{27}$, $f_{28}$) resulted in improved predictions accuracy and confidence for both bypass and reuse.
IP frame length ($f_{11}$), while valuable as a pure feature component contributing to both roles, strengthened nearly any feature component it was combined with.

As an artifact of packetizing flows into manageable units bounded by Maximum Transmission Unit (MTU), IP's frame length field was a notable indicator of packet inter-arrival patterns.
It is further noteworthy that while $f_{11}$ was able to stand alone, it also significantly strengthened when combined with role-focused feature components.
While not included in this study, the interplay between frame length and received packet size (only differing if IP fragmentation has occurred), is expected to be noteworthy low-hanging fruit in further feature design explorations.
The final feature ranking pass of our differential Information Gain approach preferred the information density of role-orthogonal feature components.

% ,  feature ranking exploration described in Section \ref{hp-fsa} preferred combinations of 
% have little active unique 
 % -- adapting to overall cache pressure.
% Related to bias?


\subsection{Automatic Throttling}
One of the critical aspects of cache management is the ability to dynamically adapt prediction aggressiveness in response to changing cache pressure.
While not quite hardened against adversarial attacks, the Hash Perceptron flow correlation mechanism presented in this work exhibits inherent self-throttling behavior which adapts to changes in cache pressure.
The correlation feedback mechanism reinforces likely good predictions, while predictions with less probability of being correct naturally tend to regress to the natural bias of the system.  See Appendix \ref{appendix:efficiency} for additional cache efficiency analysis providing insight into cache pressure dynamics.

\begin{figure}[ht] \centering
% \includegraphics[width=\linewidth]{2012-sanjose_feature-settling}
\includegraphics[width=0.9\linewidth]{2012-sanjose_feature-bias_selected}
\caption{Feature Bias}
\label{fig:hp-rank-bias}
\end{figure}

Figure \ref{fig:hp-rank-bias} shows the feature's prediction bias over epochs of each evaluated feature.
Naively, we would desire all features to be neutral biased; however, this isn't aligned with the objective of discriminating flows based on estimated short-term activity.
Features assume a role implicit by the construction of their components, producing a bias skewed towards the utility of their insight.
Pessimistic features (net bias of evict) primarily contribute to the role of bypass, effectively filtering flows from entering the cache until sufficient optimism arises from other features.
Optimistic features (net bias of keep) primarily contribute to reuses prediction.
The adaptive nature of hashed perception mechanism dynamically adjusts each feature to the average observed cache pressure.




% Due to features tending bias either to accept or reject, they can tend to be either aggressive (high TP/TN) or conservative (high FP/FN).
% Features tend to score well when observing just accuracy, false positive/negative rates.



%% this is disrupting flow.  how do i present feature roles..?
% \subsubsection{Feature Weight Distribution}



% hard to say any distribtuion is good vs bad...  Would be interesting to showcase the shapes of the best performing features vs the worst.
% can say that output distribtuion is != weight distribution (i.e. feature input is not uniform random)
% psudo mapping is availbile with just bucket counts; full trace of actual output distribution can be used to verify assumption


% \begin{figure*} [H]
% \begin{tabular}{ccc}
% \includegraphics[width=55mm]{flow-8689} & \includegraphics[width=55mm]{flow-8133259} & \includegraphics[width=55mm]{flow-201} \\
% (a) & (b) & (c) \\[6pt]
% \includegraphics[width=55mm]{flow-9612} & \includegraphics[width=55mm]{flow-1873} & \includegraphics[width=55mm]{flow-3679999} \\
% (d) & (e) & (f) \\[6pt]
% \end{tabular}
% \caption{Varios Flow Interarrival Patterns}
% \end{figure*}




% \subsubsection{Correlation Steady State}
% % Default to 5-bit saturating counters (output of each correlation table)
% The dynamics of feature table size, feature sparsity, training event rate effectively determine the hysteresis of the predictor.
% The warm-up time of the predictor can be roughly approximated through a sliding window average of feature opinion output.
% Through experimentation, we found 5-bit saturating counters offered a good trade-off in training responsiveness and accuracy.
% Feature table length also impacts the hysteresis, but less so due to the inherent sparsity of each feature input.

% \begin{figure}[H] \centering
% \includegraphics[width=0.7\linewidth]{2012-sanjose_feature-bias} 
% \caption{Feature Output Bias}
% \label{fig:hp-rank-bias}
% \end{figure}


% \subsubsection{Complementary Feature Bias}
% bypass and reuse are similar but distinct questions.  both are using the same feature tables
% most interesting observation here is if the top N features have a complementary default bias; i.e. some features are really good at knowing when reuse is likely because of past history, while others are best suited for bypass triage


% TODO: reduce aspect ratio





%%%%%%%%%%%%%%%%%%%%%
\section{Summary}
Cache management for stateful flow tables is a largely unexplored area of research, despite their wide deployment.
This work demonstrates viability of the Hashed Perceptron approach to cache management.
The Hashed Perceptron correlation technique is uniquely able to cope with noisy information sources, well suited for network flow table cache management.

% Much of the innovations in cache management are trade secrets, unique to product differentiation.

Feature creation is still an designer's art coupled with both intuitive and counter-intuitive surprises.
Early feedback and iteration is essential to enable fast design exploration.
Advancements to systematic feature ranking and selection, even if non-optimal, allow designers to focus on system architecture and feature creation first and foremost.
% Feature ranking is a complex optimization problem, 
Ultimately, any ML approach is inherently reliant on effective feature creation and information sources.

The Hashed Perceptron technique is proving to be an interesting lightweight ML approach where weights are run-time correlations, enabling adaptability beyond comparable offline techniques.
% amenible to hardware implementation... 
When applying the Hashed Perceptron technique to a new domain it became apparent how a multi-feature, consensus-based system significantly improves prediction reliability compared to hand-crafting complex heuristics.
A interesting observation in the context of network traffic is the resiliency of the Hashed Perceptron technique to cope with noisy or even misleading features.
While it is certainly possible to degrade performance, the Hashed Perceptron's ability to combine multiple features offers stability over any single perspective technique.

% with many potential applications in real-time systems.
% A hybrid approach

% The value of this work is the process of refining features.
Few mechanisms allow combining independent correlations reliably, yet efficiently to improve system performance.
This work describes the process of adapting and evaluating the Hashed Perceptron mechanism to an unexplored domain, where the input patterns and vectors available to features bring unique challenges.














